Generated Knowledge Prompting for Commonsense Reasoning

It remains an open question whether incorporating external knowledge benefits commonsense reasoning while maintaining the flexibility of pretrained sequence models. To investigate this question, we develop generated knowledge prompting, which consists of generating knowledge from a language model, then providing the knowledge as additional input when answering a question. Our method does not require task-specific supervision for knowledge integration, or access to a structured knowledge base, yet it improves performance of large-scale, state-of-the-art models on four commonsense reasoning tasks, achieving state-of-the-art results on numerical commonsense (NumerSense), general commonsense (CommonsenseQA 2.0), and scientific commonsense (QASC) benchmarks. Generated knowledge prompting highlights large-scale language models as flexible sources of external knowledge for improving commonsense reasoning. Our code is available at https://github.com/liujch1998/GKP

==> [ARR 2021.11] Generated Knowledge Prompting/atrash/analysis.tex <==
\section{Good Knowledge, and More Knowledge}
\label{sec:analysis}

\input{floats/qasc_summary}

Why Generated Knowledge Prompting works, after all?
Through the following quantitative study of the behavior of the inference model, we show that the performance boost is due to two factors: the quality of knowledge, and the max-ensembling algorithm on a diverse set of knowledge.
% We hope to provide more insight by quantitatively characterizing the behavior of the inference model under \name{}.
We choose to study the QASC dataset in particular because it comes with annotated ground knowledge, and we will focus on two metrics of the inference model: the mean and variance of the answer scores.

\textbf{Metrics.}
For each question, we generate multiple knowledge sentences.
An answer choice may be evaluated differently by the inference model when prompted with each knowledge sentence, thus inducing a list of scores: $\{ p_I(a \mid [k_m||q]) \}$.
We define \textit{induced average} and \textit{induced deviation} as the mean and standard deviation of these scores, and denote them as $\mu_K(q,a)$ and $\sigma_K(q,a)$, respectively.
Because eventually predictions are made based on only one of the prompts (selected by the max-ensembling algorithm), we also define the \textit{selected score} as the score of an answer under the selected prompt:
\begin{align*}
\omega_K(q,a) &= p_I(a \mid [\hat{k}||q])
\end{align*}
where $\hat{k} = \argmax_{k \in K_q}{\max_{a \in A_q}{p_I(a \mid [k||q])}}$.
For the vanilla inference method (i.e with no knowledge prompting), we define
\begin{align*}
\mu_\varnothing(q,a) = \omega_\varnothing(q,a) = p_I(a|q), \sigma_\varnothing(q,a) = 0
\end{align*}
Since we are interested in the general trend due to our method, we compute the mean of these metrics over the entire dataset, while making a particular distinction between correct answers and distractors:
\begin{align*}
\bar{X}^* &= \text{Mean}_{(q,a^*) \in D}[X(q,a^*)] \\
\bar{X}' &= \text{Mean}_{(q,a^*) \in D, a' \in A_q \backslash \{a^*\}}[X(q,a')]
\end{align*}
where $X \in \{ \mu, \sigma, \omega \}$.
Note that $\bar{\mu}^*$ can be viewed as a continuous proxy to the prediction accuracy under the Mixture-of-Experts ensembling algorithm (\autoref{eqn:moe}).

\textbf{Baselines.}
We consider a few alternatives to \textit{ground knowledge} as the prompt:


\textbf{Discussion.}
\autoref{fig:qasc_summary} plots the aforementioned metrics of a T5-11b inference model on the QASC dev set.

Looking at the mean of average score (the dashed lines), we conclude that
\begin{align*}
\bar{\mu}_\varnothing^* \approx \bar{\mu}_L^* &\approx \bar{\mu}_C^* < \bar{\mu}_K^* \\
\bar{\mu}_\varnothing' \approx \bar{\mu}_L' &\approx \bar{\mu}_C' > \bar{\mu}_K'
\end{align*}
This tells us that on average, prompting with the generated knowledge increases the scores for correct answers and decreases the scores for distractors, thereby improving the prediction accuracy.
In comparison, language prompting ($L$) and context prompting ($C$) do not move this metric significantly, while prompting with gold facts ($G2$ and $G1$) show similar trend as Generated Knowledge Prompting, yet with larger magnitude.
This indicates that the generated knowledge are generally effective, while with inferior quality than the gold annotated knowledge.
The better knowledge we have, the more we can help the inference model.

Next, the error bars and the mean of selected score (solid lines) show that
\begin{align*}
\bar{\sigma}_i^* > \bar{\sigma}_i' &\text{ for } i \in \{ K, C, L \} \\
\bar{\omega}_\varnothing^* \approx \bar{\omega}_L^* &< \bar{\omega}_C^* << \bar{\omega}_K^* \\
\bar{\omega}_\varnothing' \approx \bar{\omega}_L' &> \bar{\omega}_C' >> \bar{\omega}_K'
\end{align*}
(Note that the score axis uses a logistic scale, so the standard deviation is not intuitive to see.)
This tells us that the induced variance of the scores tend to be larger for correct answers than for distractors.
Since extreme scores help knowledge and answers stand out in the max-ensembling algorithm, the larger induced variance further helps correct answers to beat the distractors.
Note that this observation is also true for language prompting ($L$) and context prompting ($C$).
The combined effect of induced average and induced deviation results in an amplified boost as shown by the selected scores $\bar{\omega}$.
Having good knowledge and more knowledge are therefore both indispensable ingredients to the success of our method.

==> [ARR 2021.11] Generated Knowledge Prompting/atrash/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Performing commonsense reasoning requires commonsense knowledge.
Although pretrained language models implicitly contain a large amount of knowledge and can be directly applied for commonsense reasoning \cite{trinh2018simple, yang-etal-2020-designing}, incorporating external knowledge bases can boost performance on some of these tasks \cite{mitra2019additional, bian2021benchmarking}. % \yejin{This statement comes across as inaccurate over-claim... "usually" is too strong as it sounds like "almost always". more accurate phrasing would be "can boost ... on some of these tasks"} 
On the other hand, language models themselves can serve the role of knowledge bases as they allow for querying \textit{symbolic knowledge} (i.e. knowledge expressed as natural language statements) via conditional generation \cite{petroni-etal-2019-language, jiang-etal-2020-know}.
% \yejin{this sentence is not entirely accurate. the prior work was trying to be catchy with their titles, which we took too literally here. also, when we use the word "mine", it already implies that the source is not a KB, just raw noisy stuff mixed with other stuff... a more accurate phrasing would be "On the other hand, PLMs themselves can serve the role of knowledge bases as they allow for querying symbolic knowledge via conditional generation"}
Therefore, we explore the following question: Can we use statements of knowledge elicited from language models to improve model performance on commonsense reasoning tasks?

\input{floats/diagram}
\input{floats/qualitative}

% With the recent boom of prompt-based learning, it is widely known that a large variety of knowledge can be elicited from PLMs \cite{}.
% Also intensively studied is that incorporating external knowledge can improve the performance of LM-based inference on various tasks, including CSR \cite{}.
% Therefore, a natural research question to ask is: Are knowledge elicited from LMs themselves helpful for the LMs' inference?

We observe that model predictions on commonsense questions can be rectified when prompted with simple but relevant knowledge statements.
\autoref{fig:diagram} shows an example: the question that asks how many sides a brick has can be transformed into more explicit reasoning over a given fact, \textsl{\uline{A brick is a cube.}} (Assuming that the model readily knows that a cube has six faces.)
\autoref{tab:qualitative} shows more such examples across different datasets, with how the prediction is influenced by the additional knowledge.
In this sense, when faced with questions that requires commonsense, the model may be implicitly performing two jobs together: (1) to come up with \textit{ground knowledge}, i.e. knowledge statements that are helpful in reasoning about the question, and (2) to perform reasoning based on such knowledge.
Our hypothesis is that breaking this down into two explicit steps, namely knowledge generation and knowledge-prompted inference, would unleash the model capacity so it can focus on an explicit and knowledge-grounded reasoning procedure.
While some existing work also leverage certain types of model-generated text to improve performance on commonsense reasoning \cite{shwartz-etal-2020-unsupervised, paranjape-etal-2021-prompting, bosselut2021dynamic}, we focus on generating and prompting knowledge that can explicitly support the reasoning process in a general way.

% A few existing work have shown that PLMs can leverage certain types of text generated by themselves to improve their CSR inference performance \cite{shwartz-etal-2020-unsupervised, paranjape-etal-2021-prompting, bosselut2021dynamic}.
% However, these methods are inefficient, domain-restricted, and/or require heavy domain expertise and engineering efforts to transfer.
% We would like to have a knowledge generation process that is flexible enough to generate diverse types of knowledge, so that the generated knowledge stays relevant to the domain.
% While these methods are often built upon thinking of what kinds of knowledge \textit{can} be generated, \yejin{I am not sure this statement is a particularly accurate summary of the prior work... did prior work explore the scope of knowledge that "can be" generated?} we take a different approach by reflecting on what kinds of knowledge are \textit{needed}. \yejin{prior work compared also study what knowledge "need to be" generated in some sense. Hanna/Bhargavi's paper for example demonstrate that contrastive knowledge need to be generated? can we find a different angle that is more accurate and crisp?}
% These methods often make \textit{a priori} assumptions on the type of knowledge to generate, and use them to control the generation process, leading to knowledge that may be only loosely relevant to answering the question.
% To address this, we take an approach by first reflecting on what are the commonalities of knowledge that are the most relevant to CSR, and then proposing a generic framework that systematically generates and utilizes such knowledge across various CSR domains.
% We hypothesize that many CSR problems can be reduced to more basic types of reasoning over \textit{ground knowledge} -- sentences that can serve as the premises for some reasoning process.
% For instance, in \autoref{fig:diagram} the commonsense question, which asks how many sides a brick has, can become a deductive reasoning problem when given the premise \textsl{\uline{A brick is a cube}}. (Assuming that the model knows that a cube has six faces.)
% The examples in \autoref{tab:qualitative} show how CSR problems from various datasets can, when provided with the appropriate knowledge, be reduced to different reasoning types such as deduction, induction, analogy, and paraphrasing.
% For example, in \S\ref{sec:numersense} we show that numerical CSR problems can, when provided with the appropriate premises, be reduced to straightforward reasoning types such as deduction, induction, paraphrasing, etc.
% In this sense, when answering a CSR question, the model may be implicitly performing two jobs together: (1) to come up with the knowledge that are helpful to answering the question, and (2) to reason with such knowledge.
% Breaking this down into two explicit steps, namely knowledge generation and knowledge-augmented inference, would unleash the model capacity so it can focus on a reduced form of reasoning.

In this work, we present the Generated Knowledge Prompting framework that follows this approach.
We take the pretrained language models off-the-shelf, elicit question-related ground knowledge  from these models, and augment the question with such knowledge before sending it to the model for inference.
This process is unsupervised and resource-efficient, since we do not need a training set to finetune the knowledge generation or inference model, or an in-domain knowledge base to retrieve knowledge from.
It is also more generic and engineering-efficient compared to previous methods, making it easily adaptable to various tasks.
% Generated Knowledge Prompting would be particularly beneficial for nascent, low-resource commonsense reasoning tasks where there is no or little training data to properly finetune the model with, and no appropriate knowledge base from which to retrieve relevant knowledge.
% Such scenario is conceivable either with a new diagnostic CSR benchmark, or a production QA system where incoming user queries may not fit in the domain of any existing CSR dataset.

We apply our method on recently released commonsense reasoning datasets -- NumerSense, CommonsenseQA, CommonsenseQA 2.0, and QASC -- and demonstrate that we can push the limits of existing models. % with only lightweight engineering efforts, and without any extra data collection or model optimization steps.
Our method improves the state-of-the-art of NumerSense by about 9\%, and that of CommonsenseQA 2.0 by about 2\%.
It also shows superior performance over the state-of-the-art generative knowledge approach, self-talk \cite{shwartz-etal-2020-unsupervised}, and is comparable to retrieval-based methods.
Experimental results show that our method is effective under a variety of settings: with different sizes of knowledge generation models and inference models, and with both zero-shot and finetuned inference models.
In particular, it is effective even when knowledge generation and inference are done with the same base language model.

% So does Generated Knowledge Prompting work so well for the reason we think it does?
% That is to say, are the generated knowledge truly providing grounds for reasoning?
% \name{} can be perceived as a type of symbolic knowledge transfer if we use the knowledge generated by a larger model to improve a smaller inference model.
% However, it is not very intuitive as to why performance also improves when knowledge generation and inference are done with the same model.
% If knowledge are encoded implicitly in the neural components of the PLM, how come generating them symbolically be helpful for inference?
% To understand this, we conduct a quantitative study of the behavior of the inference model (\S\ref{sec:analysis}).
Through a quantitative study of the behavior of the inference model (\S\ref{sec:analysis}), we find that two factors contribute to the method's success: the high quality of the generated knowledge, and ensembling over the predictions of many knowledge statements.
Furthermore, qualitative analysis (\S\ref{sec:qualitative}) also shows that the generated knowledge can reduce commonsense question answering to certain explicit reasoning procedures using the generated knowledge. % serves to reduce the reasoning process in ways that we expected, and even enables new reasoning types that we did not anticipate.
% Our intuition is that by explicating ground knowledge through symbolic generation, the model can incorporate the knowledge with full certainty and thus perform more deterministic knowledge-grounded reasoning.
% We hope that the insights we share will inspire further efforts on improving the robustness and explainability of PLM-based inference.
Our work shows a novel yet important role of symbolic representation of knowledge in the neural reasoning process, and we hope that the insights we share will inspire further efforts on neuro-symbolic knowledge integration.

==> [ARR 2021.11] Generated Knowledge Prompting/atrash/numersense.tex <==
\section{A Case Study with Numerical Commonsense}
\label{sec:numersense}

\alisainline{There should be a table that shows examples of generated knowledge for each dataset. This has the benefit of giving an example from each dataset to illustrate the task, as well as showing what model's generative capabilities are. I think it would be a good Page 2 table, even if it's referenced much later on in the experiments.}

We first conduct a case study on the NumerSense dataset \cite{lin-etal-2020-birds} to show how ground knowledge prompts models to perform better on commonsense inference.%, and how we can generate such relevant knowledge.

NumerSense challenges models on the task of numerical commonsense reasoning.
It presents generic statements about common concepts while masking a number token in each sentence, which the model needs to recover.
The masked numbers are always integers between zero and ten (inclusive), so NumerSense can be formulated as a multiple-choice task.

We analyze a strong baseline model on NumerSense based on T5-11B.
Although it achieves a very high performance on the leaderboard, this model still makes numerous mistakes on very simple questions.
Consider the following question from the dev set:
\begin{center}\textbf{Most motorcycles have [M] tires.}\end{center}
T5-11B predicts \textcolor{wrong}{four} as an answer with a confidence of \textcolor{wrong}{0.33}, whereas the correct answer \textcolor{right}{two} only gets a confidence of \textcolor{right}{0.32}.
However, if we prepend the following knowledge sentences to this question:
\begin{center}\textsl{A motorcycle has two wheels. Each wheel has a tire.}\end{center}
The inference model then assigns a high confidence (\textcolor{right}{0.86}) to the correct answer \textcolor{right}{two} and thus make the right prediction.
Note that the question and the context form a deductive reasoning process, where the question is the conclusion and the two additional sentences serve as the premises.
The addition of knowledge essentially reduces this commonsense problem to a deductive reasoning problem.
Furthermore, we observe that using only one of these two premises as the context is also able to rectify the prediction (\autoref{tab:numersense_qual}), demonstrating that the inference model can incorporate partially-complete premise set into its reasoning process.

Based on the question of interest, there can be different kinds of ground knowledge, and they can transform the type of reasoning required in different ways.
\autoref{tab:numersense_qual} shows more examples where manually-written knowledge rectifies the prediction.
Ground knowledge can be numerical (e.g. \textsl{\uline{A cube has eight vertices.}}), attributive (e.g. \textsl{\uline{Triangles are polygons with the least number of sides.}}), and taxonomical (e.g. \textsl{\uline{Scallop is a kind of clam.}}).
The reduced reasoning types may be straightforward paraphrasing, logical reasoning such as deduction and induction, numerical reasoning such as counting and arithmetics, etc.

With this observation, we pose the next research question: can we use models to generate ground knowledge that are still able to rectify the model predictions?
In the next section, we introduce a framework for knowledge generation and prompting which answers this question with a resounding yes.

==> [ARR 2021.11] Generated Knowledge Prompting/atrash/qasc_hist.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{floats/qasc_hist.png}
\caption{
    Distribution of some metrics of inference probabilities under different input augmentation methods.
    This is an alternative view of \autoref{fig:qasc_scatter}.
    We compute the mean and standard deviation of inference probabilities under all augmentation texts for each example, and plot a histogram of these metrics across all examples (the first and second rows, respectively).
    We also plot a histogram of the inference probability under the selected augmentation text for each example (the third row).
    The (\textcolor{right}{green} and \textcolor{wrong}{red}) solid vertical lines stand for the mean of these metrics, whereas the dashed vertical lines are the mean of such metrics on the no-augmentation baseline.
}
\label{fig:qasc_hist}
\end{figure*}

==> [ARR 2021.11] Generated Knowledge Prompting/atrash/qasc_scatter.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{floats/qasc_scatter.png}
\caption{
    Impact of input augmentation methods on inference probabilities.
    Each plot is a scatter plot that shows the change in inference probability with some input augmentation method.
    The horizontal axis is the inference probability without input augmentation, and the vertical axis is the inference probability with an augmentation text.
    We plot the impact of each augmentation text on every example in the QASC dev set.
    The \textcolor{yellow}{yellow} dots show all $M$ augmentations for each example, and the \textcolor{right}{green} or \textcolor{wrong}{red} dots show the augmentation selected by the max-ensembling algorithm to make the final prediction.
    The first row of plots show the impact on \textcolor{right}{correct answers}, whereas the second row show the impact on \textcolor{wrong}{distractors}.
    We present results for the following input augmentation methods: Language Augmentation, Context Augmentation, and Knowledge Augmentation with model-generated knowledge or gold knowledge.
    We use $M=20$ for methods with model-generated augmentations, and $M=1$ or $2$ for methods using gold knowledge as augmentations.
    The legend shows the mean inference probability.
    The right-most column of plots is special: it shows the impact of finetuning instead of input augmentation. 
    The vertical axis is the inference probability from a finetuned T5-11b model with no input augmentation.
}
\label{fig:qasc_scatter}
\end{figure*}

==> [ARR 2021.11] Generated Knowledge Prompting/atrash/qasc_summary.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{floats/qasc_summary.png}
\caption{
    Inference model behavior under different types of prompts.
    Measured on the QASC dev set with T5-11b as the inference model.
    Generated Knowledge Prompting is denoted by Knowledge ($K$), whereas other types of prompts are described in \S\ref{sec:analysis}.
    For each type of prompt, we show the mean of induced average (dashed lines), mean of induced deviation (filled areas), and selected score (solid lines) for \textcolor{right}{correct answers} and \textcolor{wrong}{distractors}.
    We also plot the \textcolor{blue}{prediction accuracy} given by the inference model.
}
\label{fig:qasc_summary}
\end{figure*}

==> [ARR 2021.11] Generated Knowledge Prompting/atrash/qual_numersense.tex <==
\begin{table*}[t]
\footnotesize
\centering
\begin{tabular}{p{9.5cm}|ccc}
\toprule
\textbf{Question} / \textsl{Knowledge} & \textbf{Prediction} & \textbf{Confidence} & \textbf{Reasoning} \\
\midrule
\textbf{most motorcycles have [M] tires.} & \textcolor{wrong}{four} & \textcolor{wrong}{0.33} | \textcolor{right}{0.32} & CSR \\
\qquad \textsl{Each wheel has a tire.} & \textcolor{right}{two} & \textcolor{right}{0.53} & Deduction \\
\qquad \textsl{A motorcycle has two wheels.} & \textcolor{right}{two} & \textcolor{right}{0.70} & Deduction \\
\qquad \textsl{A motorcycle has two wheels. Each wheel has a tire.} & \textcolor{right}{two} & \textcolor{right}{0.86} & Deduction \\
\midrule
\textbf{any closed two-dimensional shape must have at least [M] sides.} & \textcolor{wrong}{two} & \textcolor{wrong}{0.27} | \textcolor{right}{0.18} & CSR \\
\qquad \textsl{Triangles are polygons with the least number of sides.} & \textcolor{right}{three} & \textcolor{right}{0.85} & Deduction \\
\midrule
\textbf{clams have evolved to have [M] shells.} & \textcolor{wrong}{no} & \textcolor{wrong}{0.37} | \textcolor{right}{0.18} & CSR \\
\qquad \textsl{Scallop is a kind of clam. A scallop has two shells.} & \textcolor{right}{two} & \textcolor{right}{0.53} & Induction \\
\midrule
\textbf{a normal cube has [M] corners.} & \textcolor{wrong}{six} & \textcolor{wrong}{0.47} | \textcolor{right}{0.15} & CSR \\
\qquad \textsl{A cube has eight vertices.} & \textcolor{right}{eight} & \textcolor{right}{0.40} & Paraphrasing \\
\midrule
\textbf{a game of chess may have [M] outcomes.} & \textcolor{wrong}{two} & \textcolor{wrong}{0.48} | \textcolor{right}{0.08} & CSR \\
\qquad \textsl{In a game of chess, we can win, or lose, or draw with the opponent.} & \textcolor{right}{three} & \textcolor{right}{0.51} & Counting \\
\midrule
\textbf{a proton is made of [M] independent quarks.} & \textcolor{wrong}{six} & \textcolor{wrong}{0.34} | \textcolor{right}{0.30} & CSR \\
\qquad \textsl{A proton is made of two up quarks and one down quark.} & \textcolor{right}{three} & \textcolor{right}{0.92} & Arithmetic \\
\bottomrule
\end{tabular}
\caption{
    Examples from NumerSense dev set where additional knowledge rectifies the prediction.
    The first row of each section is the original question and the inference results associated with it, followed by manually-written knowledge text that are prepended before the question during inference.
    We show \textcolor{right}{correct predictions in green}, \textcolor{wrong}{incorrect predictions in red}, and their corresponding confidence values produced by the model.
}
\label{tab:numersense_qual}
\end{table*}

==> [ARR 2021.11] Generated Knowledge Prompting/atrash/results.tex <==
\begin{table*}[t]
% \footnotesize
\centering
\begin{tabular}{c|ccc|c|cc|cc}
\toprule
\textbf{Task} & \multicolumn{3}{c}{\textbf{NumerSense}} & \textbf{CSQA} & \multicolumn{2}{c}{\textbf{CSQA2}} & \multicolumn{2}{c}{\textbf{QASC}} \\
\midrule
Inference & \multicolumn{3}{c}{T5-11b} & T5-11b & \multicolumn{2}{c}{Unicorn-11b-ft} & \multicolumn{2}{c}{T5-11b} \\
& \textit{dev} & \textit{test-core} & \textit{test-all} & \textit{dev} & \textit{dev} & \textit{test} & \textit{dev} & \textit{test} \\
\midrule
\textbf{Baseline} & 67.5 & 70.23 & 64.08 & 39.89 & 69.9 & 70.2 & 48.16 & 44.89 \\
\rowcolor{ours}
\textbf{ours} & \textbf{78.0} & \textbf{79.24} & \textbf{72.47} & \textbf{47.26} & \textbf{72.37} & \textbf{73.03} & \textbf{58.32} & \textbf{55.00} \\
\bottomrule
\end{tabular}
\caption{
    An overview of empirical results across all tasks.
    \textbf{ours}: Generated Knowledge Prompting, which is highlighted in green (same below).
    For our method, knowledge are generated by GPT3 for all datasets.
    All tasks use the off-the-shelf T5-11b model for inference, except for CSQA2 where we use a finetuned version of Unicorn-11b.
}
\label{tab:results}
\end{table*}

==> [ARR 2021.11] Generated Knowledge Prompting/atrash/results_csqa.tex <==
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{cc|c}
\toprule
\multicolumn{3}{c}{\textbf{CSQA}} \\
\midrule
\textbf{Inference} & \textbf{Knowledge} & \textbf{dev} \\
\midrule
T5-11b & -- & 39.89 \\
T5-11b & self-talk (GPT3) & 45.37 \\
\rowcolor{ours}
T5-11b & GPT3 & \textbf{47.26} \\
\midrule
UQA-11b & -- & 76.99 \\
UQA-11b & self-talk (GPT3) & 77.97 \\
\rowcolor{ours}
UQA-11b & GPT3 & \textbf{78.71} \\
% \midrule
% T5-11b-ft & -- & 83.54 & \textcolor{red}{TODO} \\
% T5-11b-ft & GPT3 & \textbf{83.78} & \textcolor{red}{TODO} \\
% \midrule
% UQA-11b-ft & -- & 85.18 & \textcolor{red}{TODO} \\
% UQA-11b-ft & GPT3 & \textbf{85.34} & \textcolor{red}{TODO} \\
\midrule
\multicolumn{2}{c}{Prev. SOTA$^\ddagger$} & 81.8 \\
\bottomrule
\end{tabular}
\caption{
    Detailed empirical results on CSQA.
    \textbf{UQA}: the UnifiedQA model.
    $\ddagger$: ALBERT + SFR (prev. SOTA with no reference to ConceptNet).
}
\label{tab:results_csqa}
\end{table}

==> [ARR 2021.11] Generated Knowledge Prompting/atrash/results_csqa2.tex <==
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{cc|cc}
\toprule
\multicolumn{4}{c}{\textbf{CSQA2}} \\
\midrule
\textbf{Inference} & \textbf{Knowledge} & \textbf{dev} & \textbf{test} \\
\midrule
Unicorn-11b-ft & --$^\ddagger$ & 69.9$^\ddagger$ & 70.2$^\ddagger$ \\
\rowcolor{ours}
Unicorn-11b-ft & GPT3 & \textbf{72.37} & \textbf{73.03} \\
\midrule
Unicorn-11b-ft & Google snippets$^\dagger$ & 74.0$^\dagger$ & 73.3$^\dagger$ \\
\bottomrule
\end{tabular}
\caption{
    Detailed empirical results on CSQA2.
    $\ddagger$: Finetuned Unicorn-11b baseline by \citet{talmor2021commonsenseqa} (prev. SOTA without Google retrieval).
    $\dagger$: Knowledge prompting with Google-retrieved snippets \cite{talmor2021commonsenseqa}.
}
\label{tab:results_csqa2}
\end{table}

==> [ARR 2021.11] Generated Knowledge Prompting/atrash/results_numersense.tex <==
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{cc|ccc}
\toprule
\multicolumn{5}{c}{\textbf{NumerSense}} \\
\midrule
\textbf{Inference} & \textbf{Knowledge} & \textbf{dev} & \textbf{test-core} & \textbf{test-all} \\
\midrule
T5-11b & --$^{*}$ & 67.5 & 70.23$^{*}$ & 64.08$^{*}$ \\
T5-11b & IR$^{\dagger}$ & -- & 70.41$^{\dagger}$ & 65.10$^{\dagger}$ \\
\multicolumn{2}{c}{Prev. SOTA$^{\ddagger}$} & -- & 72.61$^{\ddagger}$ & 66.18$^{\ddagger}$ \\
\rowcolor{ours}
T5-11b & GPT3 & \textbf{78.0} & \textbf{79.24} & \textbf{72.47} \\
\midrule
GPT3 & -- & 72.0 & 74.91 & 66.34 \\
\rowcolor{ours}
GPT3 & GPT3 & \textbf{81.0} & \textbf{80.74} & \textbf{73.46} \\
\bottomrule
\end{tabular}
\caption{
    Detailed empirical results on NumerSense with different knowledge sources and inference models.
    *: T5-11b baseline \cite{stanford}.
    $\dagger$: Information retrieval method \cite{uscink}.
    $\ddagger$: Submission by ISI Waltham.
    Leaderboard retrieved on 09/09/2021.
}
\label{tab:results_numersense}
\end{table}

==> [ARR 2021.11] Generated Knowledge Prompting/atrash/results_qasc.tex <==
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{cc|cc}
\toprule
\multicolumn{4}{c}{\textbf{QASC}} \\
\midrule
\textbf{Inference} & \textbf{Knowledge} & \textbf{dev} & \textbf{test} \\
\midrule
T5-11b & -- & 48.16 & 44.89 \\
\rowcolor{ours}
T5-11b & GPT3 & \textbf{58.32} & \textbf{55.00} \\
\midrule
UQA-11b & -- & 67.93 & 67.07 \\
\rowcolor{ours}
UQA-11b & GPT3 & \textbf{74.41} & \textbf{75.33} \\
\midrule
T5-11b-ft & -- & 76.03 & 73.91 \\
\rowcolor{ours}
T5-11b-ft & GPT3 & \textbf{78.62} & \textbf{77.17} \\
\midrule
UQA-11b-ft & -- & 81.75 & 76.74 \\
\rowcolor{ours}
UQA-11b-ft & GPT3 & \textbf{84.02} & \textbf{80.33} \\
\midrule
\multicolumn{2}{c}{Prev. SOTA$^\ddagger$} & -- & 89.57 \\
\bottomrule
\end{tabular}
\caption{
    Detailed empirical results on QASC.
    \textbf{UQA}: the UnifiedQA model.
    $\ddagger$: UQA-11b-ft + IR (prev. SOTA).
}
\label{tab:results_qasc}
\end{table}

==> [ARR 2021.11] Generated Knowledge Prompting/atrash/theory.tex <==
\section{A Theoretical Perspective}

In this section, we make an attempt to explain why knowledge augmentation works so well.
We will present some theories, and show quantitative analysis with QASC in support of these theories.

The method we will look at is Input Augmentation (IA), which is a generalization of UKA and contains two weaker alternatives to it: Context Augmentation (CA) and Language Augmentation (LA).
All these method involves extending the input with a piece of text.
The difference is that the augmentation text in CA and LA may not be as relevant as UKA.
In particular, CA augments the input with a piece of text sampled from the context of the input, and LA does so by freely sampling some text from the language model without conditioning on the input.
We introduce these alternatives as they provide simpler mathematical interface than UKA.

\subsection{Preliminaries}

Suppose we have a dataset $D = \{(x, y)\}$, where $x \in X$ is the input text and $y \in Y$ is the desired output text, and an inference language model $p(y|x)$.
The model decides the best output with $\hat{y} = \argmax_{y \in Y}{p(y|x)}$.

During IA, we prepend a piece of text $z \in Z$ before the input $x$, so that the inference process can be written as $p(y|z,x)$.
In practice, a set of augmentation texts $Z_e$ are sampled, and prediction results produced by augmenting each $z \in Z_e$ are ensembled to derive the final prediction:
\begin{align*}
z^* &= \argmax_{z \in Z_e}{\max_{y \in Y}{p(y|z,x)}} \\
\hat{y} &= \argmax_{y \in Y}{p(y|z^*,x)}
\end{align*}

Conceptually, $X = Y = Z = L$, where $L$ is the space of natural language texts.
We will use this setting for our theoretical analysis.
However, for empirical analysis with the QASC dataset, we restrict $Y = Y_q$, the list of choices for each question in QASC, and $Z = Z_e$ because it is intractable to marginalize over the entire text space.
We normalize the inference probabilities over the reduced output space:
\begin{align*}
\tilde{p}(y|x) &= \frac{p(y|x)}{\sum_{y' \in Y_q}{p(y'|x)}} \\
\tilde{p}(y|z,x) &= \frac{p(y|z,x)}{\sum_{y' \in Y_q}{p(y'|z,x)}}
\end{align*}

\subsection{An assumption with language models}

For simplicity, assume that we work with an autoregressive LM.
We define the joint probability and conditional probability of pairs of texts w.r.t. the LM as
\begin{align*}
p(x,y) &\equiv p([x || y]) \\
p(y|x) &\equiv \frac{p(x,y)}{p(x)} \equiv \frac{p([x || y])}{p(x)}
\end{align*}

We make the assumption that the LM satisfies the following equation:
\begin{align*}
p(a) &= \sum_{b \in L}{p(b) p(a|b)} \equiv \sum_{b \in L}{p(b,a)} \equiv \sum_{b \in L}{p([b || a])}
\end{align*}
This is the foundation of our theoretical analysis below.
I guess this is not strictly true for LMs, and we need to look into how close it is to real LMs, but I suppose this provides a reasonable approximation that greatly simplifies our further discussion.

\subsection{Language and Context Augmentation}

For a given example $(x, y) \in D$, in Language Augmentation we arbitrarily sample the augmentation text from the LM: $z \sim p(\cdot)$; whereas in Context Augmentation we sample it from the context (a.k.a. continuation) of the input: $z \sim p(\cdot|x)$.

\subsubsection{Conservation of expectation of inference probabilities}
\label{sec:expectation}

For Context Augmentation, the expectation of probability assigned by the inference model to the desired output is equal to that without IA.
Formally,
\begin{align*}
p(y|x) &= \sum_{z \in L}{p(z|x) p(y|z,x)} = \mathbb{E}_{z \sim p(\cdot|x)}{\big[ p(y|z,x) \big]}
\end{align*}
This also applies to the desired output $y$ any distractor $y' \in L$.
Therefore, if only one augmentation text is generated, Context Augmentation does not improve the model's confidence on the correct answer on average.

\textcolor{red}{TODO: Similar result for LAug?}

% Note, however, that if we compute the expectation of model loss (i.e. negative log likelihood, NLL), Context Augmentation is guaranteed to increase the loss value:
% \begin{align*}
% L(y;x) &= -\log{p(y|x)} \\
% &= -\log{\sum_{z \in L}{p(z|x) p(y|z,x)}} \\
% &\le \sum_{z \in L}{p(z|x) \big[ -\log{p(y|z,x)} \big]} & \text{(Jensen's inequality)} \\
% &= \mathbb{E}_{z \sim p(\cdot|x)}{\big[ L(y;z,x) \big]}
% \end{align*}
% which does not give us a stable baseline to investigate the effect of input augmentation, so we do not use this metric.

\subsubsection{(Differential) increase of variance of inference probabilities}
\label{sec:variance}

Although LA and CA are shown not to make the inference model more confident on the desired outputs, they can create an intrinsic variance within such confidence by introducing multiple augmentation texts.
The naive inference process assigns a single confidence score to each output for a given input: $p(y|x)$.
In comparison, IA produces a list of confidence scores:
\begin{align*}
\big[ p(y|z_1,x), \hdots, p(y|z_m,x), \hdots, p(y|z_M,x) \big]
\end{align*}
where $Z_e = \{z_1, \hdots, z_M\}$.

Through the quantitative analysis, we will empirically show that the variance of these confidence scores tends to be larger for desired outputs than distractors:
\begin{align*}
\mathbb{E}_{(x,y),Z_e}{\Big[\text{Std}\big[\{p(y|z_i,x)\}\big]\Big]} \\
> \mathbb{E}_{(x,y),y',Z_e}{\Big[\text{Std}\big[\{p(y'|z_i,x)\}\big]\Big]}
\end{align*}
One hypothesis is that, for desired outputs, the evidences/explanations/justifications in support of these outputs can make reasoning more convincing.\footnote{Though this also means that those evidence in contradiction with these outputs are more convincing as well.}

As a result, desired outputs tend to contain more \textit{extreme} confidence values under IA.
This implies that the max-ensembling algorithm, which uses the augmentation that most strongly supports any output, tends to pick up augmentations that result in high confidence values on the desired output.

\subsubsection{Reduction of entropy in output space}
\label{sec:entropy}

Now we take a look at the change of entropy of output space due to IA.
The entropy of output space without IA is $\mathcal{H}(Y|x)$, and the entropy with IA is $\mathcal{H}(Y|Z,x)$.
The change is equal to
\begin{align*}
\mathcal{H}(Y|Z,x) - \mathcal{H}(Y|x) &= -\mathcal{I}(Y;Z|x)
\end{align*}
which is the mutual information of output variable $Y$ and augmentation variable $Z$ for a given input $x$.

For LA, $Z \sim p(\cdot)$ is sampled freely from the LM, so it has zero mutual information with $Y$.
Therefore, LA does not change the entropy of output space.

For CA, $Z \sim p(\cdot|x)$ is sampled conditioning on the input $x$, so $Z$ is correlated to $Y$, and thus the mutual information $\mathcal{I}(Y;Z|x)$ is positive.
Therefore, CA reduces the entropy of output space.

\subsection{Quantitative analysis on QASC}

\input{floats/results_qasc_hierarchy}
\input{floats/qasc_scatter}
\input{floats/qasc_hist}

In QASC, each example comes with a fact sentence that can directly answer the question; this sentence is in turn formed by the composition of two separate \textit{fact} sentences, which are also provided in the dataset.
In some sense, these sentences can be regarded as the best possible augmentations, so that we can see the upperbound of capability of IA.

We run inference on the QASC dev set with the off-the-shelf T5-11b and UnifiedQA-T5-11b models, using the following input augmentation methods:
\begin{enumerate}
\item Language Augmentation. For each example, we use GPT2-large to sample $M=20$ random sentences, without looking at the content of question or choices.
\item Context Augmentation. For each example, we use GPT2-large to sample $M=20$ continuations to the question. The generated sentences can be seen as a representative set of context sentences wrt the question sentence.
\item Knowledge Augmentation. For each example, we use GPT3 to generate up to $M=20$ knowledge sentences based on the keywords in the question, using a few-shot, in-context learning prompt.
\item Knowledge Augmentation with gold, separate knowledge. In this case we use the two \textit{fact} sentences associated with the question as augmentation texts, and thus $M=2$.
\item Knowledge Augmentation with gold, combined knowledge. In this case we use the composition \textit{fact} sentence associated with the question as augmentation texts, and thus $M=1$.
\end{enumerate}

\autoref{fig:qasc_scatter} shows the impact of these input augmentation methods on inference probabilities for correct answers and distractors.
See the caption for explanation of these plots.
Ideally, we would like to see points to fall into the upper-left triangle for correct answers, and into the lower-right triangle for distractors, which would manifest that we are pushing the model to be more confident on correct answers.
The plots for finetuned T5 inference model clearly shows such a trend, where the dots in the answer plot (first row) are densely aggregated around the $y=1$ line, and the dots in the distractor plot (second row) around the $y=0$ line.
KA with gold facts, either separate or combined, also shows a similar trend, and the average of inference probabilities moves accordingly (up for correct answers, down for distractors).
If we focus on the \textcolor{right}{green} and \textcolor{wrong}{red} dots, which shows the impact of the augmentation text selected by the max-ensembling algorithm, the trend is even more apparent, and the magnitude of change in average model confidence is also magnified.
This proves the effectiveness of IA when working with best possible augmentation text -- the upperbound is high.

For KA with model-generated augmentation texts, we see the same trend with milder magnitude -- the average inference probabilities still change considerably while not as much as KA with oracle augmentation texts.
LA and CA, on the other hand, show no significant change on average inference probabilities when considering all augmentation texts, which is consistent with our theory in \S\ref{sec:expectation}.
Interestingly, if we only consider the selected augmentation texts, there is still an improvement to the inference probabilities over the baseline.

We observe that IA methods tend to create more extreme inference probabilities.
The dots tend to be pushed towards the upper ($y=1$) and lower ($y=0$) areas of the plots, whereas the area in the middle is relatively sparse.
The existence of such phenomenon indirectly manifests the reduction of entropy in output space in \S\ref{sec:entropy}.
This phenomenon is stronger for correct answer than for distractors, which is mentioned in \S\ref{sec:variance}.
Also, this phenomenon is stronger for selected augmentation texts.

Perhaps the differential increase of variance of inference probabilities is more evident in \autoref{fig:qasc_hist}.
The second row plots the distribution of standard deviation of inference probabilities induced by augmentation.
As we can see, under all input augmentation methods, the induced variance tend to be larger for correct answers than distractors.

\subsection{Summary}

\input{floats/theory_summary}

\autoref{tab:theory_summary} summarizes our findings, namely:
\begin{enumerate}
\item Language and Context Augmentation does not change the expectation of inference probabilities. However, empirical results show that Knowledge Augmentation tends to increase the model's confidence on desired outputs (i.e. correct answers), and decrease the model's confidence on undesired outputs (i.e. distractors).
\item Input Augmentation methods create an intrinsic variance on the inference probabilities. Empirical results show that this variance tends to be larger for desired outputs than undesired outputs. This, together with our max-ensembling algorithm, makes the desired outputs more favorable for the inference model.
\item Input Augmentation methods reduce the entropy of the output space. Though this does not guarantee that the desired outputs get more favorited than undesired outputs.
\end{enumerate}

==> [ARR 2021.11] Generated Knowledge Prompting/atrash/theory_summary.tex <==
\begin{table}[t]
\centering
\begin{tabular}{c|cc|cc|c}
\toprule
\textbf{Method} & \multicolumn{2}{c}{\textbf{$\mu$}} & \multicolumn{2}{c}{\textbf{$\sigma$}} & \textbf{$\mathcal{H}$} \\
& \textbf{\cmark} & \textbf{\xmark} & \textbf{\cmark} & \textbf{\xmark} & \\
\midrule
Language Augmentation & \multicolumn{2}{c}{--} & \textcolor{magenta}{$\uparrow$}$\uparrow$ & \textcolor{magenta}{$\uparrow$} & \textcolor{magenta}{--} \\
Context Augmentation & \multicolumn{2}{c}{\textcolor{magenta}{--}} & \textcolor{magenta}{$\uparrow$}$\uparrow$ & \textcolor{magenta}{$\uparrow$} & \textcolor{magenta}{$\downarrow$} \\
Knowlegde Augmentation & $\uparrow$ & $\downarrow$ & \textcolor{magenta}{$\uparrow$}$\uparrow$ & \textcolor{magenta}{$\uparrow$} & \textcolor{magenta}{$\downarrow$} \\
\bottomrule
\end{tabular}
\caption{
    Summary of UKA theory and quantitative analysis.
    Black means observed in empirical results but have no theoretical proof; \textcolor{magenta}{magenta} means both observed in empirical results and we have a theoretical proof.
}
\label{tab:theory_summary}
\end{table}

==> [ARR 2021.11] Generated Knowledge Prompting/floats/diagram.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{floats/diagram.png}
\caption{
    % Inference with a standard language model produces a distribution over answer candidates given a query (top).
    % Top: Standard models select the highest probability prediction without reference to symbolic knowledge.
    % Bottom: Generated knowledge prompting  involves (i) generating question-specific symbolic knowledge, (ii) using the knowledge statement which best supports answering the question under the inference model.
    % maximizes prediction probability during inference. 
    % Illustrating Generated Knowledge Prompting.
    % Top: Standard language model inference.
    % Bottom: Inference with Generated Knowledge Prompting.
    Generated knowledge prompting involves (i) using few-shot demonstrations to generate question-related knowledge statements from a language model; 
    % (ii) prompting a language model with the generated knowledge to integrate them into predictions.
    (ii) using a second language model to make predictions with each knowledge statement, then selecting the highest-confidence prediction.
}
\label{fig:diagram}
\end{figure}

==> [ARR 2021.11] Generated Knowledge Prompting/floats/guidelines.tex <==
\begin{table*}
\footnotesize
\centering
\begin{tabular}{l p{2.5cm} p{10cm}}
\toprule
\textbf{Attribute} & \textbf{Options} & \textbf{Description and Examples} \\
\midrule
\textbf{Grammaticality} & grammarical; ungrammatical but understandable; completely gibberish & Whether the knowledge statement is grammatical. We are aware that some of the statements are not fully grammatical. If you can still understand what the statement says, even if it's an incomplete sentence or slightly ungrammatical, please select the "ungrammatical but understandable" option. \\
\midrule
\textbf{Relevance} & relevant; not relevant & Whether a knowledge statement is relevant to the given question. A statement is relevant if it covers one the same topics as the question, or contains a salient concept that is same or similar to one in the question. Examples: \\
\\
& & \textcolor{red}{[Question]} you may take the subway back and forth to work <mask> days a week. \\
& & \textcolor{orange}{[Knowledge]} You take the subway back and forth to work five days a week. \\
& & \textcolor{blue}{[Judgment]} Relevant, because the question and knowledge are both about the topic of business days. \\
\\
& & \textcolor{red}{[Question]} a bradypus torquatus is native to brazil and has <mask> toes on each limb. \\
& & \textcolor{orange}{[Knowledge]} A bradypus torquatus is a kind of mammal. A mammal has four limbs. \\
& & \textcolor{blue}{[Judgment]} Relevant, because the question and knowledge share a common salient concept "bradypus torquatus". \\
\midrule
\textbf{Factuality} & factual; not factual & Whether a knowledge statement is (mostly) factually correct or not. If there are exceptions or corner cases, it can still be considered factual if they are rare or unlikely. Examples: \\
\\
& & \textcolor{orange}{[Knowledge]} A limousine has four doors. \\
& & \textcolor{blue}{[Judgment]} Factual. \\
\\
& & \textcolor{orange}{[Knowledge]} A human hand has four fingers and a thumb. \\
& & \textcolor{blue}{[Judgment]} Factual, despite that there are exceptions -- people with disabilities may have less or more fingers. \\
\\
& & \textcolor{orange}{[Knowledge]} A rectangle is a shape with two equal sides. \\
& & \textcolor{blue}{[Judgment]} Not factual, because a rectangle has four sides. \\
\midrule
\end{tabular}
\caption{Human evaluation guidelines. Continued in \autoref{tab:guidelines_2}.}
\label{tab:guidelines}
\end{table*}

\begin{table*}
\footnotesize
\centering
\begin{tabular}{l p{2.5cm} p{10cm}}
\toprule
\textbf{Attribute} & \textbf{Options} & \textbf{Description and Examples} \\
\midrule
\textbf{Helpfulness} & helpful; neutral; harmful & Whether a knowledge statement provides useful information in support OR contradiction of the answer. A statement is helpful if it supports the answer either directly or indirectly. More on indirect support -- The statement might not directly answer the question directly, yet it may support an indirect reasoning path that reaches the answer. A statement is harmful if it negates the answer or supports an alternative potential answer either directly or indirectly. A statement is neutral if it is neither helpful nor harmful. Examples: \\
\\
& & \textcolor{red}{[Question]} you may take the subway back and forth to work <mask> days a week. \\
& & \textcolor{green}{[Answer]} five \\
& & \textcolor{orange}{[Knowledge]} You take the subway back and forth to work five days a week. \\
& & \textcolor{blue}{[Judgment]} Helpful. Because the statement directly supports the answer. \\
\\
& & \textcolor{red}{[Question]} spiders have <mask> legs. \\
& & \textcolor{green}{[Answer]} eight \\
& & \textcolor{orange}{[Knowledge]} Arachnids have eight legs. \\
& & \textcolor{blue}{[Judgment]} Helpful. Although the statement does not directly refer to spiders, together with the fact that "spiders are a kind of arachnids" it completes a reasoning chain in deriving the answer. \\
\\
& & \textcolor{red}{[Question]} a game of chess may have <mask> outcomes. \\
& & \textcolor{green}{[Answer]} three \\
& & \textcolor{orange}{[Knowledge]} A game of chess has two outcomes. \\
& & \textcolor{blue}{[Judgment]} Harmful. Since the statement supports answering "two" instead of "three". \\
\\
& & \textcolor{red}{[Question]} a bradypus torquatus is native to brazil and has <mask> toes on each limb. \\
& & \textcolor{green}{[Answer]} three \\
& & \textcolor{orange}{[Knowledge]} A bradypus torquatus is a kind of mammal. A mammal has four limbs. \\
& & \textcolor{blue}{[Judgment]} Neutral. The statement does not provide information in favor or contrast of the answer. \\
\bottomrule
\end{tabular}
\caption{(continued) Human evaluation guidelines.}
\label{tab:guidelines_2}
\end{table*}

==> [ARR 2021.11] Generated Knowledge Prompting/floats/human.tex <==
\begin{figure*}[t]
\begin{minipage}{.4\linewidth}
\centering
\includegraphics[width=\linewidth]{floats/human_bar.png}
\end{minipage}
\hfill
\begin{minipage}{.58\linewidth}
\centering
\includegraphics[width=\linewidth]{floats/human_pie.png}
\end{minipage}
\caption{
    Human evaluation of generated knowledge.
    \textbf{Left:} Percentage of good knowledge statements along each axis.
    \textbf{Right:} Agreement between human and machine on helpfulness of selected knowledge.
}
\label{fig:human}
\end{figure*}

==> [ARR 2021.11] Generated Knowledge Prompting/floats/methods.tex <==
\begin{table*}[b]
\footnotesize
\centering
\begin{tabular}{ccc}
\toprule
\textbf{Method} & \textbf{Knowledge Generator} & \textbf{Inference Model} \\
\midrule
\textbf{CAGE} \cite{rajani-etal-2019-explain} & task-finetuned & joint-finetuned \\
\citet{latcinnik2020explaining} & task-finetuned & joint-finetuned \\
\textbf{DynaGen} \cite{bosselut2021dynamic} & task-finetuned & joint-finetuned \\
\textbf{Self-talk} \cite{shwartz-etal-2020-unsupervised} & template-prompted & 0-shot \\
\textbf{Contrastive expl.} \cite{paranjape-etal-2021-prompting} & template-prompted & 0-shot \& joint-finetuned \\
\midrule
\textbf{Generated knowledge prompting} (ours) & demonstrations-prompted & 0-shot \& task-finetuned \\
\bottomrule
\end{tabular}
\caption{
    Comparison of methods that add generated text to an inference model.
    \textbf{Knowledge Generator}: \textit{task-finetuned} -- a model finetuned to generate task-specific knowledge; \textit{template-prompted} -- an off-the-shelf LM from which knowledge statements are elicited via templates; \textit{demonstration-prompted} -- an off-the-shelf LM from which knowledge statements are elicited via few-shot demonstrations (\S\ref{sec:method_generation}).
    \textbf{Inference Model}: \textit{0-shot} -- an off-the-shelf LM that is set up to make predictions; \textit{task-finetuned} -- a model finetuned with task training data (and without seeing extra knowledge); \textit{joint-finetuned} -- a model finetuned with task training data \textit{and} generated knowledge.
}
\label{tab:methods}
\end{table*}

==> [ARR 2021.11] Generated Knowledge Prompting/floats/prompt.tex <==
\begin{table*}[t]
\footnotesize
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{rp{7.5cm}p{8cm}}
\textbf{Task} & \textbf{NumerSense} & \textbf{QASC} \\
\midrule
\textbf{Prompt} & Generate some numerical facts about objects. Examples: & Generate some knowledge about the input. Examples: \\
\addlinespace[4pt]
& Input: \textbf{penguins have <mask> wings.} & Input: \textbf{What type of water formation is formed by clouds?} \\
& Knowledge: \textit{Birds have two wings. Penguin is a kind of bird.} & Knowledge: \textit{Clouds are made of water vapor.} \\
\addlinespace[4pt]
& ... & ... \\
\addlinespace[4pt]
& Input: \textbf{a typical human being has <mask> limbs.} & Input: \textbf{The process by which genes are passed is} \\
& Knowledge: \textit{Human has two arms and two legs.} & Knowledge: \textit{Genes are passed from parent to offspring.} \\
\addlinespace[4pt]
& Input: \textbf{\{question\}} & Input: \textbf{\{question\}} \\
& Knowledge: & Knowledge:
\end{tabular}
}
\caption{
    Prompts for knowledge generation for two of our tasks, NumerSense and QASC. 
    The prompt consists of an instruction, five demonstrations of question-knowledge pairs, and a new question placeholder.
    For full prompts on all the tasks we evaluate on, see Appendix \ref{sec:prompts}.
}
\label{tab:prompt}
\end{table*}

==> [ARR 2021.11] Generated Knowledge Prompting/floats/prompt_csqa.tex <==
\begin{table*}[h!]
\footnotesize
\centering
\begin{tabular}{r|p{12cm}}
\textbf{Task} & \textbf{Prompt} \\ % & \textbf{Reasoning} \\
CSQA & Generate some knowledge about the concepts in the input. Examples:\\
\\
& Input: \textbf{Google Maps and other highway and street GPS services have replaced what?} \\ % & \textcolor{gray}{Commonsense} \\
& Knowledge: \textit{Electronic maps are the modern version of paper atlas.} \\ % & Deduction \\
\\
& Input: \textbf{The fox walked from the city into the forest, what was it looking for?} \\ % & \textcolor{gray}{Commonsense} \\
& Knowledge: \textit{Natural habitats are usually away from cities.} \\ % & Deduction \\
\\
& Input: \textbf{You can share files with someone if you have a connection to a what?} \\ % & \textcolor{gray}{Commonsense} \\
& Knowledge: \textit{Files can be shared over the Internet.} \\ % & Paraphrasing \\
\\
& Input: \textbf{Too many people want exotic snakes.  The demand is driving what to carry them?} \\ % & \textcolor{gray}{Commonsense} \\
& Knowledge: \textit{Some people raise snakes as pets.} \\ % & Deduction \\
\\
& Input: \textbf{The body guard was good at his duties, he made the person who hired him what?} \\ % & \textcolor{gray}{Commonsense} \\
& Knowledge: \textit{The job of body guards is to ensure the safety and security of the employer.} \\ % & Paraphrasing \\
\\
& Input: \textbf{\{question\}}\\
& Knowledge:
\end{tabular}
\caption{
    Prompt for knowledge generation on CSQA.
    Demonstration examples are selected from the CSQA training set; we manually write relevant knowledge for each input question.
}
\label{tab:prompt_csqa}
\end{table*}

==> [ARR 2021.11] Generated Knowledge Prompting/floats/prompt_csqa2.tex <==
\begin{table*}[h]
\footnotesize
\centering
\begin{tabular}{r|p{12cm}}
\textbf{Task} & \textbf{Prompt} \\
CSQA2 & Generate some knowledge about the input. Examples:\\
\\
& Input: \textbf{Greece is larger than mexico.}\\
& Knowledge: \textit{Greece is approximately 131,957 sq km, while Mexico is approximately 1,964,375 sq km, making Mexico 1,389\% larger than Greece.}\\
\\
& Input: \textbf{Glasses always fog up.}\\
& Knowledge: \textit{Condensation occurs on eyeglass lenses when water vapor from your sweat, breath, and ambient humidity lands on a cold surface, cools, and then changes into tiny drops of liquid, forming a film that you see as fog. Your lenses will be relatively cool compared to your breath, especially when the outside air is cold.}\\
\\
& Input: \textbf{A fish is capable of thinking.}\\
& Knowledge: \textit{Fish are more intelligent than they appear. In many areas, such as memory, their cognitive powers match or exceed those of 'higher' vertebrates including non-human primates. Fish's long-term memories help them keep track of complex social relationships.}\\
\\
& Input: \textbf{A common effect of smoking lots of cigarettes in one's lifetime is a higher than normal chance of getting lung cancer.}\\
& Knowledge: \textit{Those who consistently averaged less than one cigarette per day over their lifetime had nine times the risk of dying from lung cancer than never smokers. Among people who smoked between one and 10 cigarettes per day, the risk of dying from lung cancer was nearly 12 times higher than that of never smokers.}\\
\\
& Input: \textbf{A rock is the same size as a pebble.}\\
& Knowledge: \textit{A pebble is a clast of rock with a particle size of 4 to 64 millimetres based on the Udden-Wentworth scale of sedimentology. Pebbles are generally considered larger than granules (2 to 4 millimetres diameter) and smaller than cobbles (64 to 256 millimetres diameter).}\\
\\
& Input: \textbf{\{question\}}\\
& Knowledge:
\end{tabular}
\caption{
    Prompt for knowledge generation on CSQA2.
    Demonstration examples are selected from the CSQA2 training set; we use the annotated \textit{Google featured snippet} as the knowledge.
}
\label{tab:prompt_csqa2}
\end{table*}

==> [ARR 2021.11] Generated Knowledge Prompting/floats/prompt_numersense.tex <==
\begin{table*}[h!]
\footnotesize
\centering
\begin{tabular}{r|p{10cm}}
\textbf{Task} & \textbf{Prompt} \\ % & \textbf{Reasoning} \\
NumerSense & Generate some numerical facts about objects. Examples:\\
\\
& Input: \textbf{penguins have <mask> wings.} \\ % & \textcolor{gray}{Commonsense} \\
& Knowledge: \textit{Birds have two wings. Penguin is a kind of bird.} \\ % & Deduction \\
\\
& Input: \textbf{a parallelogram has <mask> sides.} \\ % & \textcolor{gray}{Commonsense} \\
& Knowledge: \textit{A rectangular is a parallelogram. A square is a parallelogram.} \\ % & Induction \\
\\
& Input: \textbf{there are <mask> feet in a yard.} \\ % & \textcolor{gray}{Commonsense} \\
& Knowledge: \textit{A yard is three feet.} \\ % & Paraphrasing \\
\\
& Input: \textbf{water can exist in <mask> states.} \\ % & \textcolor{gray}{Commonsense} \\
& Knowledge: \textit{There states for matter are solid, liquid, and gas.} \\ % & Counting \\
\\
& Input: \textbf{a typical human being has <mask> limbs.} \\ % & \textcolor{gray}{Commonsense} \\
& Knowledge: \textit{Human has two arms and two legs.} \\ % & Arithmetics \\
\\
& Input: \textbf{\{question\}}\\
& Knowledge:
\end{tabular}
\caption{
    Prompt for knowledge generation on NumerSense.
    Demonstration examples are manually written and the knowledge enables explicit reasoning procedures to answer the input question. % represent different types of reasoning reduction.
    % The reasoning type annotations in the table are not part of the prompt.
}
\label{tab:prompt_numersense}
\end{table*}

==> [ARR 2021.11] Generated Knowledge Prompting/floats/prompt_qasc.tex <==
\begin{table*}[h]
\footnotesize
\centering
\begin{tabular}{r|p{12cm}}
\textbf{Task} & \textbf{Prompt} \\ % & \textbf{Reasoning} \\
QASC & Generate some knowledge about the input. Examples:\\
\\
& Input: \textbf{What type of water formation is formed by clouds?} \\ % & \textcolor{gray}{Commonsense} \\
& Knowledge: \textit{Clouds are made of water vapor.} \\ % & Deduction \\
\\
& Input: \textbf{What can prevent food spoilage?} \\ % & \textcolor{gray}{Commonsense} \\
& Knowledge: \textit{Dehydrating food is used for preserving food.} \\ % & Paraphrasing \\
\\
& Input: \textbf{The process by which genes are passed is} \\ % & \textcolor{gray}{Commonsense} \\
& Knowledge: \textit{Genes are passed from parent to offspring.} \\ % & Deduction \\
\\
& Input: \textbf{The stomach does what in the body?} \\ % & \textcolor{gray}{Commonsense} \\
& Knowledge: \textit{The stomach is part of the digestive system.} \\ % & Paraphrasing \\
\\
& Input: \textbf{What can cause rocks to break down?} \\ % & \textcolor{gray}{Commonsense} \\
& Knowledge: \textit{Mechanical weathering is when rocks are broken down by mechanical means.} \\ % & Deduction \\
\\
& Input: \textbf{\{question\}}\\
& Knowledge:
\end{tabular}
\caption{
    Prompt for knowledge generation on QASC.
    Demonstration examples are selected from the QASC training set; we use one of the gold separate facts as the knowledge.
}
\label{tab:prompt_qasc}
\end{table*}

==> [ARR 2021.11] Generated Knowledge Prompting/floats/qualitative.tex <==
\begin{table*}[t]
\footnotesize
\centering
\begin{tabular}{cp{7cm}ccc}
\toprule
\textbf{Dataset} & \textbf{Question} / \textsl{Knowledge} & \textbf{Prediction} & \textbf{Score} & \textbf{Reasoning} \\
\midrule
\multirow{2}{*}{NumerSense} & \textbf{clams have evolved to have [M] shells.} & \textcolor{wrong}{no} & \textcolor{wrong}{0.37} | \textcolor{right}{0.18} & \textcolor{gray}{Commonsense} \\
& \qquad \textsl{Clams have a bivalve shell.} & \textcolor{right}{two} & \textcolor{right}{0.89} & Paraphrasing \\
\midrule
\multirow{2}{*}{NumerSense} & \textbf{an easel can have [M] or four legs.} & \textcolor{wrong}{two} & \textcolor{wrong}{0.45} | \textcolor{right}{0.45} & \textcolor{gray}{Commonsense} \\
& \qquad \textsl{A tripod is a kind of easel.} & \textcolor{right}{three} & \textcolor{right}{0.46} & Induction \\
% \midrule
% \multirow{2}{*}{NumerSense} & \textbf{bricks are [M] sided.} & \textcolor{wrong}{four} & \textcolor{wrong}{0.27} | \textcolor{right}{0.13} & \textcolor{gray}{Commonsense} \\
% & \qquad \textsl{A brick is a cube.} & \textcolor{right}{six} & \textcolor{right}{0.71} & Deduction \\
% \midrule
% \multirow{2}{*}{NumerSense} & \textbf{the word children means [M] or more kids.} & \textcolor{wrong}{one} & \textcolor{wrong}{0.37} | \textcolor{right}{0.35} & \textcolor{gray}{Commonsense} \\
% & \qquad \textsl{The word child means one kid.} & \textcolor{right}{two} & \textcolor{right}{0.91} & Analogy \\
\midrule
\multirow{2}{*}{CSQA} & \textbf{Where does a heifer's master live?} & \textcolor{wrong}{slaughter house} & \textcolor{wrong}{0.89} | \textcolor{right}{0.01} & \textcolor{gray}{Commonsense} \\
& \qquad \textsl{The master of a heifer is a farmer.} & \textcolor{right}{farm house} & \textcolor{right}{0.92} & Deduction \\
\midrule
\multirow{2}{*}{CSQA} & \textbf{Aside from water and nourishment what does your dog need?} & \textcolor{wrong}{walked} & \textcolor{wrong}{0.55} | \textcolor{right}{0.04} & \textcolor{gray}{Commonsense} \\
& \qquad \textsl{Dogs need attention and affection.} & \textcolor{right}{lots of attention} & \textcolor{right}{0.91} & Elimination \\
% \midrule
% \multirow{2}{*}{CSQA} & \textbf{What is the result of applying for job?} & \textcolor{wrong}{praise} & \textcolor{wrong}{0.98} | \textcolor{right}{0.02} & \textcolor{gray}{Commonsense} \\
% & \qquad \textsl{The result of applying for a job is that you get a job.} & \textcolor{right}{being employed} & \textcolor{right}{0.99} & Paraphrasing \\
\midrule
\multirow{2}{*}{CSQA} & \textbf{I did not need a servant. I was not a what?} & \textcolor{wrong}{in charge} & \textcolor{wrong}{0.47} | \textcolor{right}{0.32} & \textcolor{gray}{Commonsense} \\
& \qquad \textit{People who have servants are rich.} & \textcolor{right}{rich person} & \textcolor{right}{0.99} & Abduction \\
\midrule
\multirow{2}{*}{CSQA2} & \textbf{Part of golf is trying to get a higher point total than others.} & \textcolor{wrong}{yes} & \textcolor{wrong}{1.00} | \textcolor{right}{0.00} & \textcolor{gray}{Commonsense} \\
& \qquad \textit{The player with the lowest score wins.} & \textcolor{right}{no} & \textcolor{right}{1.00} & Negation \\
% \midrule
% \multirow{2}{*}{CSQA2} & \textbf{If a piece of lead and a feather are falling thought vacuum, none will reach the bottom earlier.} & \textcolor{wrong}{no} & \textcolor{wrong}{0.59} | \textcolor{right}{0.41} & \textcolor{gray}{Commonsense} \\
% & \qquad \textit{All objects fall at the same rate in a vacuum.} & \textcolor{right}{yes} & \textcolor{right}{1.00} & Deduction \\
% \midrule
% \multirow{2}{*}{CSQA2} & \textbf{A minute will pass only if sixty seconds have passed.} & \textcolor{wrong}{no} & \textcolor{wrong}{1.00} | \textcolor{right}{0.00} & \textcolor{gray}{Commonsense} \\
% & \qquad \textit{A minute is a unit of time equal to 60 seconds.} & \textcolor{right}{yes} & \textcolor{right}{1.00} & Paraphrasing \\
\midrule
\multirow{2}{*}{CSQA2} & \textbf{Eighth plus eight is smaller than fifteen.} & \textcolor{wrong}{yes} & \textcolor{wrong}{0.97} | \textcolor{right}{0.03} & \textcolor{gray}{Commonsense} \\
& \qquad \textit{Eighth plus eight is sixteen, which is larger than fifteen.} & \textcolor{right}{no} & \textcolor{right}{1.00} & Numerical \\
\midrule
\multirow{2}{*}{QASC} & \textbf{[M] is used for transportation.} & \textcolor{wrong}{plastic} & \textcolor{wrong}{0.41} | \textcolor{right}{0.12} & \textcolor{gray}{Commonsense} \\
& \qquad \textit{Bicycles are used for transportation.} & \textcolor{right}{boats} & \textcolor{right}{0.74} & Analogy \\
% \midrule
% \multirow{2}{*}{QASC} & \textbf{Hydrostatic skeletons are a feature of some [M].} & \textcolor{wrong}{eukaryotic cells} & \textcolor{wrong}{0.46} | \textcolor{right}{0.06} & \textcolor{gray}{Commonsense} \\
% & \qquad \textit{Hydrostatic skeletons are a feature of some fish.} & \textcolor{right}{aquatic animals} & \textcolor{right}{0.96} & Induction \\
% \midrule
% \multirow{2}{*}{QASC} & \textbf{[M] requires studying the weather.} & \textcolor{wrong}{research} & \textcolor{wrong}{0.48} | \textcolor{right}{0.43} & \textcolor{gray}{Commonsense} \\
% & \qquad \textit{Meteorology is the study of the weather.} & \textcolor{right}{meteorology} & \textcolor{right}{1.00} & Paraphrasing \\
% \midrule
% \multirow{2}{*}{QASC} & \textbf{Knowledge of the stars can be used for [M].} & \textcolor{wrong}{life} & \textcolor{wrong}{0.63} | \textcolor{right}{0.16} & \textcolor{gray}{Commonsense} \\
% & \qquad \textit{Navigation is when people use the stars to find their way.} & \textcolor{right}{travel} & \textcolor{right}{0.89} & Deduction \\
\bottomrule
\end{tabular}
\caption{
    More examples where prompting with generated knowledge reduces the reasoning type and rectifies the prediction.
    The first row of each section is the original question and the inference results associated with it; the second row is a model-generated knowledge statement that prompts the inference model.
    We show \textcolor{right}{correct answers in green}, \textcolor{wrong}{incorrect answers in red}, and their corresponding scores assigned by the inference model.
}
\label{tab:qualitative}
\end{table*}

==> [ARR 2021.11] Generated Knowledge Prompting/floats/qualitative_short.tex <==
\begin{table*}[t]
\footnotesize
\centering
\begin{tabular}{cp{7cm}ccc}
\toprule
\textbf{Dataset} & \textbf{Question} / \textsl{Knowledge} & \textbf{Prediction} & \textbf{Reasoning} \\
% \midrule
% \multirow{2}{*}{NumerSense} & \textbf{clams have evolved to have [M] shells.} & \textcolor{wrong}{no} & \textcolor{wrong}{0.37} | \textcolor{right}{0.18} & \textcolor{gray}{Commonsense} \\
% & \qquad \textsl{Clams have a bivalve shell.} & \textcolor{right}{two} & \textcolor{right}{0.89} & Paraphrasing \\
\midrule
\multirow{2}{*}{NumerSense} & \textbf{an easel can have [M] or four legs.} & \textcolor{wrong}{two} & \textcolor{gray}{Commonsense} \\
& \qquad \textsl{A tripod is a kind of easel.} & \textcolor{right}{three} & Induction \\
% \midrule
% \multirow{2}{*}{NumerSense} & \textbf{bricks are [M] sided.} & \textcolor{wrong}{four} & \textcolor{wrong}{0.27} | \textcolor{right}{0.13} & \textcolor{gray}{Commonsense} \\
% & \qquad \textsl{A brick is a cube.} & \textcolor{right}{six} & \textcolor{right}{0.71} & Deduction \\
% \midrule
% \multirow{2}{*}{NumerSense} & \textbf{the word children means [M] or more kids.} & \textcolor{wrong}{one} & \textcolor{wrong}{0.37} | \textcolor{right}{0.35} & \textcolor{gray}{Commonsense} \\
% & \qquad \textsl{The word child means one kid.} & \textcolor{right}{two} & \textcolor{right}{0.91} & Analogy \\
\midrule
\multirow{2}{*}{CSQA} & \textbf{Where does a heifer's master live?} & \textcolor{wrong}{slaughter house} & \textcolor{gray}{Commonsense} \\
& \qquad \textsl{The master of a heifer is a farmer.} & \textcolor{right}{farm house} & Deduction \\
% \midrule
% \multirow{2}{*}{CSQA} & \textbf{Aside from water and nourishment what does your dog need?} & \textcolor{wrong}{walked} & \textcolor{wrong}{0.55} | \textcolor{right}{0.04} & \textcolor{gray}{Commonsense} \\
% & \qquad \textsl{Dogs need attention and affection.} & \textcolor{right}{lots of attention} & \textcolor{right}{0.91} & Elimination \\
% \midrule
% \multirow{2}{*}{CSQA} & \textbf{What is the result of applying for job?} & \textcolor{wrong}{praise} & \textcolor{wrong}{0.98} | \textcolor{right}{0.02} & \textcolor{gray}{Commonsense} \\
% & \qquad \textsl{The result of applying for a job is that you get a job.} & \textcolor{right}{being employed} & \textcolor{right}{0.99} & Paraphrasing \\
\midrule
\multirow{2}{*}{CSQA} & \textbf{I did not need a servant. I was not a what?} & \textcolor{wrong}{in charge} & \textcolor{gray}{Commonsense} \\
& \qquad \textit{People who have servants are rich.} & \textcolor{right}{rich person} & Abduction \\
% \midrule
% \multirow{2}{*}{CSQA2} & \textbf{Part of golf is trying to get a higher point total than others.} & \textcolor{wrong}{yes} & \textcolor{wrong}{1.00} | \textcolor{right}{0.00} & \textcolor{gray}{Commonsense} \\
% & \qquad \textit{The player with the lowest score wins.} & \textcolor{right}{no} & \textcolor{right}{1.00} & Negation \\
% \midrule
% \multirow{2}{*}{CSQA2} & \textbf{If a piece of lead and a feather are falling thought vacuum, none will reach the bottom earlier.} & \textcolor{wrong}{no} & \textcolor{wrong}{0.59} | \textcolor{right}{0.41} & \textcolor{gray}{Commonsense} \\
% & \qquad \textit{All objects fall at the same rate in a vacuum.} & \textcolor{right}{yes} & \textcolor{right}{1.00} & Deduction \\
% \midrule
% \multirow{2}{*}{CSQA2} & \textbf{A minute will pass only if sixty seconds have passed.} & \textcolor{wrong}{no} & \textcolor{wrong}{1.00} | \textcolor{right}{0.00} & \textcolor{gray}{Commonsense} \\
% & \qquad \textit{A minute is a unit of time equal to 60 seconds.} & \textcolor{right}{yes} & \textcolor{right}{1.00} & Paraphrasing \\
% \midrule
% \multirow{2}{*}{CSQA2} & \textbf{Eighth plus eight is smaller than fifteen.} & \textcolor{wrong}{yes} & \textcolor{wrong}{0.97} | \textcolor{right}{0.03} & \textcolor{gray}{Commonsense} \\
% & \qquad \textit{Eighth plus eight is sixteen, which is larger than fifteen.} & \textcolor{right}{no} & \textcolor{right}{1.00} & Numerical \\
\midrule
\multirow{2}{*}{QASC} & \textbf{[M] is used for transportation.} & \textcolor{wrong}{plastic} & \textcolor{gray}{Commonsense} \\
& \qquad \textit{Bicycles are used for transportation.} & \textcolor{right}{boats} & Analogy \\
% \midrule
% \multirow{2}{*}{QASC} & \textbf{Hydrostatic skeletons are a feature of some [M].} & \textcolor{wrong}{eukaryotic cells} & \textcolor{wrong}{0.46} | \textcolor{right}{0.06} & \textcolor{gray}{Commonsense} \\
% & \qquad \textit{Hydrostatic skeletons are a feature of some fish.} & \textcolor{right}{aquatic animals} & \textcolor{right}{0.96} & Induction \\
% \midrule
% \multirow{2}{*}{QASC} & \textbf{[M] requires studying the weather.} & \textcolor{wrong}{research} & \textcolor{wrong}{0.48} | \textcolor{right}{0.43} & \textcolor{gray}{Commonsense} \\
% & \qquad \textit{Meteorology is the study of the weather.} & \textcolor{right}{meteorology} & \textcolor{right}{1.00} & Paraphrasing \\
% \midrule
% \multirow{2}{*}{QASC} & \textbf{Knowledge of the stars can be used for [M].} & \textcolor{wrong}{life} & \textcolor{wrong}{0.63} | \textcolor{right}{0.16} & \textcolor{gray}{Commonsense} \\
% & \qquad \textit{Navigation is when people use the stars to find their way.} & \textcolor{right}{travel} & \textcolor{right}{0.89} & Deduction \\
\bottomrule
\end{tabular}
\caption{
    More examples where prompting with generated knowledge reduces the reasoning type and rectifies the prediction.
    The first row of each section is the original question and the inference results associated with it; the second row is a model-generated knowledge statement that prompts the inference model.
    We show \textcolor{right}{correct answers in green}, \textcolor{wrong}{incorrect answers in red}, and their corresponding scores assigned by the inference model.
}
\label{tab:qualitative_short}
\end{table*}

==> [ARR 2021.11] Generated Knowledge Prompting/floats/results.tex <==
\begin{table*}[t]
\setlength{\tabcolsep}{3pt}
% \footnotesize
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c l uuu v w xx yy zz}
& & \multicolumn{3}{c}{$A$} & \multicolumn{1}{c}{$B_1$} & \multicolumn{1}{c}{$B_2$} & \multicolumn{2}{c}{$C$} & \multicolumn{2}{c}{$D_1$} & \multicolumn{2}{c}{$D_2$} \\
\toprule
& \textbf{Dataset} & \multicolumn{3}{c}{\textbf{NumerSense}} & \multicolumn{1}{c}{\textbf{CSQA}} & \multicolumn{1}{c}{\textbf{CSQA}} & \multicolumn{2}{c}{\textbf{CSQA2}} & \multicolumn{2}{c}{\textbf{QASC}} & \multicolumn{2}{c}{\textbf{QASC}} \\
& \textbf{Inference Model} & \multicolumn{3}{c}{T5-11b} & \multicolumn{1}{c}{T5-11b} & \multicolumn{1}{c}{UQA-11b-ft} & \multicolumn{2}{c}{Unicorn-ft} & \multicolumn{2}{c}{T5-11b} & \multicolumn{2}{c}{UQA-11b-ft} \\
& & dev & test$_{\text{core}}$ & test$_{\text{all}}$ & dev & dev & dev & test & dev & test & dev & test \\
\midrule
\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Knowledge Gen.}}} & ($\varnothing$) Vanilla baseline & 67.5 & 70.23 & 64.05 & 39.89 & 85.18 & 69.9 & 70.2$^{\dagger}$ & 48.16 & 44.89 & 81.75 & 76.74 \\
& ($R$) Random sentences & 68.5 & -- & -- & 21.79 & \textbf{85.42} & 70.37 & -- & 49.35 & -- & 82.18 & -- \\
& ($C$) Context sentences & \uline{70.5} & -- & -- & 42.51 & \uline{85.34} & 70.92 & -- & 55.83 & -- & 82.61 & -- \\
& ($T$) Template-based & -- & -- & -- & \uline{45.37} & -- & -- & -- & -- & -- & -- & -- \\
& ($\mathit{IR}$) Retrieval-based & -- & \uline{70.41} & \uline{65.10}$^{**}$ & -- & -- & \textbf{74.0} & \textbf{73.3}$^{\dagger\dagger}$ & \textbf{76.89} & -- & \textbf{90.06} & -- \\
& ($A$) Answers & 73.0 & -- & -- & 51.84 & 84.93 & 69.22 & -- & 52.48 & -- & 81.53 & -- \\
& ($K$) Ours & \textbf{78.0} & \textbf{79.24} & \textbf{72.47} & \textbf{47.26} & \uline{85.34} & \uline{72.37} & \uline{73.03} & \uline{58.32} & 55.00 & \uline{84.02} & 80.33 \\
\midrule
& prev. SOTA (no IR) & -- & 72.61 & 66.18$^*$ & -- & 79.1 (test)$^{\#}$ & 69.9 & 70.2$^{\dagger}$ & -- & -- & 81.75 & 76.74$^{\ddagger}$ \\
& Few-shot GPT-3 Infer. & 60.5 & -- & -- & -- & 71.58 & 53.80 & -- & -- & -- & 66.09 & -- \\
\bottomrule
\end{tabular}
}%
\caption{
    Experimental results of applying different knowledge generation methods on various tasks and inference models.
    % We report prediction accuracy in the following formats: \textbf{NumerSense} -- dev | test-core | test-all; \textbf{CSQA} -- dev; \textbf{CSQA2} and \textbf{QASC} -- dev | test.
    T5-11b is the zero-shot inference model, whereas other inference models are finetuned based on T5-11b.
    We \textbf{bold} the best and \uline{underline} the second best numbers.
    Previous SOTA and retrieval-based methods are also based on the inference model in their corresponding column:
    * T5-11b 1.1 +digits (Submission by ISI Waltham);
    ** T5-11b + IR \cite{uscink};
    \# UQA-11b-ft \cite{khashabi-etal-2020-unifiedqa} (SOTA of single-model methods without referencing ConceptNet);
    $\dagger$ Unicorn-ft \cite{talmor2021commonsenseqa};
    $\dagger\dagger$ Unicorn-ft + Google snippets \cite{talmor2021commonsenseqa};
    $\ddagger$ UQA-11b-ft \cite{khashabi-etal-2020-unifiedqa}.
}
\label{tab:results}
\end{table*}

==> [ARR 2021.11] Generated Knowledge Prompting/floats/results_numersense_knowledge.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{floats/knowledge.png}
\caption{
    Improvement by different sizes of knowledge generation model (Numersense dev set, T5-11b inference model).
}
\label{fig:results_numersense_knowledge}
\end{figure}

==> [ARR 2021.11] Generated Knowledge Prompting/floats/results_numersense_size.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{floats/inference.png}
\caption{
    Improvement on top of different sizes of inference model (Numersense dev set).
}
\label{fig:results_numersense_size}
\end{figure}

% \begin{table}[t]
% \footnotesize
% \centering
% \begin{tabular}{lccc}
% \toprule
% \multicolumn{4}{c}{\textbf{NumerSense-dev}} \\
% \midrule
% \textbf{Inference} & \textbf{Baseline} & \textbf{+Knowledge} & \textbf{$\Delta$} \\
% \midrule
% GPT-3 (175B) & 72.0 & 81.0 & +9.0 \\
% T5-11b (11B) & 67.5 & 78.0 & +10.5 \\
% T5-3b (2.8B) & 55.5 & 75.0 & +19.5 \\
% T5-large (770M) & 43.5 & 73.5 & +30.0 \\
% T5-base (220M) & 33.0 & 63.0 & +30.0 \\
% T5-small (60M) & 23.0 & 55.0 & +32.0 \\
% \bottomrule
% \end{tabular}
% \caption{
%     Improvement on different sizes of inference models.
%     Measured on Numersense dev set with the GPT-3 knowledge model.
% }
% \label{tab:results_numersense_size}
% \end{table}

==> [ARR 2021.11] Generated Knowledge Prompting/floats/results_qasc_ensembling.tex <==
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{cc}
\toprule
\textbf{Integration method} & \textbf{QASC-dev} \\
\midrule
ours & \textbf{58.32} \\
Mixture-of-Experts & 56.26 \\
Product-of-Experts & 55.94 \\
\bottomrule
\end{tabular}
\caption{
    Performance with different knowledge integration methods
    (QASC dev set, T5-11b inference model).
}
\label{tab:results_qasc_ensembling}
\end{table}

==> [ARR 2021.11] Generated Knowledge Prompting/floats/results_qasc_hierarchy.tex <==
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{clc}
\toprule
& \textbf{Knowledge Generation} & \textbf{QASC-dev} \\
\midrule
$\varnothing$ & vanilla baseline & 48.16  \\
$R$ & Random sentences & 48.70 \\
$C$ & Context sentences & 51.30 \\
$K$ & ours & \textbf{58.32} \\
\midrule
$G2$ & Gold separate facts & 76.89 \\
$G1$ & Gold combined facts & 88.55 \\
\bottomrule
\end{tabular}
\caption{
    Performance with different knowledge generation methods.
    Measured on QASC dev set with T5-11b inference model.
}
\label{tab:results_qasc_hierarchy}
\end{table}

==> [ARR 2021.11] Generated Knowledge Prompting/floats/results_qasc_quantity.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{floats/quantity.png}
\caption{
    Performance with different number of generated knowledge statements per question (QASC dev set, T5-11b inference model).
}
\label{fig:results_qasc_quantity}
\end{figure}

% \begin{table}[t]
% \footnotesize
% \centering
% \begin{tabular}{cc}
% \toprule
% \textbf{Knowledge Quantity ($M$)} & \textbf{QASC-dev} \\
% \midrule
% 0 & 48.16 \\
% 1 & 56.05 \\
% 2 & 56.59 \\
% 5 & 57.67 \\
% 10 & 57.78 \\
% 20 & \textbf{58.32} \\
% \bottomrule
% \end{tabular}
% \caption{
%     Performance with different number of generated knowledge statements per question.
%     Measured on QASC dev set with the T5-11b inference model. % \hanna{This can be a graph or a bar chart? I think a graph would be nice.}
% }
% \label{tab:results_qasc_quantity}
% \end{table}

==> [ARR 2021.11] Generated Knowledge Prompting/floats/results_sota.tex <==
\begin{table}[t]
\setlength{\tabcolsep}{3pt}
\footnotesize
\centering
\begin{tabular}{ccccc}
\toprule
& \textbf{Inference} & \textbf{Knowledge} & \textbf{dev} & \textbf{test} \\
\midrule
\multirow{2}{*}{\textbf{NS}} & T5-11b & ours & \textbf{78.0} & \textbf{79.24} | \textbf{72.47} \\
& \multicolumn{2}{c}{Prev. SOTA (no IR)$^*$} & -- & 72.61 | 66.18 \\
& \multicolumn{2}{c}{IR SOTA$^{**}$} & -- & 70.41 | 65.10 \\
\midrule
\multirow{2}{*}{\textbf{CSQA}} & UQA-11b-ft & ours & 85.34 & -- \\
& \multicolumn{2}{c}{Prev. SOTA$^{\#}$} & -- & 79.1 \\
\midrule
\multirow{2}{*}{\textbf{CSQA2}} & Unicorn-ft & ours & \textbf{72.37} & \textbf{73.03} \\
& \multicolumn{2}{c}{Prev. SOTA (no IR)$^\dagger$} & 69.9 & 70.2 \\
& \multicolumn{2}{c}{IR SOTA$^{\dagger\dagger}$} & 74.0 & 73.3 \\
\midrule
\multirow{2}{*}{\textbf{QASC}} & UQA-11b-ft & ours & \textbf{84.02} & \textbf{80.33} \\
& \multicolumn{2}{c}{Prev. SOTA (no IR)$^\ddagger$} & 81.75 & 76.74 \\
& \multicolumn{2}{c}{IR SOTA$^{\ddagger\ddagger}$} & -- & 89.57 \\
\bottomrule
\end{tabular}
\caption{
\hanna{Texts in tables are not well aligned; you should use l (instead of c) for text-based columns Here, you can remove the knowledge column; just use the column as }
    Comparison with state-of-the-art.
    For NumerSense (\textbf{NS}), the test set result consists of two splits: test-core and test-all.
    *: T5-11b 1.1 +digits (Submission by ISI Waltham).
    **: T5-11b + IR \cite{uscink}.
    \#: UQA-11b-ft \cite{khashabi-etal-2020-unifiedqa} (SOTA of single-model methods without referencing ConceptNet).
    $\dagger$: Unicorn-ft \cite{talmor2021commonsenseqa}.
    $\dagger\dagger$: Unicorn-ft + Google snippets \cite{talmor2021commonsenseqa}.
    $\ddagger$: UQA-11b-ft \cite{khashabi-etal-2020-unifiedqa}.
    $\ddagger\ddagger$: UQA-11b-ft + IR \cite{khashabi-etal-2020-unifiedqa}.  \hanna{Not clear if these are fine-tuned or zero shot; also it seems that all the infernece model sizes are similar to your T5-11b, right? then, mention it.}
}
\label{tab:results_sota}
\end{table}

==> [ARR 2021.11] Generated Knowledge Prompting/floats/results_supervised.tex <==
\begin{table}[t]
\setlength{\tabcolsep}{4pt}
\footnotesize
\centering
\begin{tabular}{clccc}
\toprule
& \textbf{Inference} & \textbf{Knowledge} & \textbf{dev} & \textbf{test} \\
\midrule
\multirow{6}{*}{\textbf{CSQA}} & \multirow{2}{*}{UQA-11b} & -- & 76.99 & -- \\
& & ours & \textbf{78.71} & -- \\
\cmidrule{2-5}
& \multirow{2}{*}{T5-11b-ft} & -- & 83.54 & -- \\
& & ours & \textbf{83.78} & -- \\
\cmidrule{2-5}
& \multirow{2}{*}{UQA-11b-ft} & -- & 85.18 & -- \\
& & ours & \textbf{85.34} & -- \\
\midrule
\multirow{2}{*}{\textbf{CSQA2}} & \multirow{2}{*}{Unicorn-ft} & --$^\dagger$ & 69.9 & 70.2 \\
& & ours & \textbf{72.37} & \textbf{73.03} \\
\midrule
\multirow{6}{*}{\textbf{QASC}} & \multirow{2}{*}{UQA-11b} & -- & 67.93 & 67.07 \\
& & ours & \textbf{74.41} & \textbf{75.33} \\
\cmidrule{2-5}
& \multirow{2}{*}{T5-11b-ft} & -- & 76.03 & 73.91 \\
& & ours & \textbf{78.62} & \textbf{77.17} \\
\cmidrule{2-5}
& \multirow{2}{*}{UQA-11b-ft} & -- & 81.75 & 76.74 \\
& & ours & \textbf{84.02} & \textbf{80.33} \\
\bottomrule
\end{tabular}
\caption{
    Improvement on finetuned models.
    \textbf{-ft}: model finetuned on the corresponding dataset.
    $\dagger$: Unicorn-ft baseline of CSQA2 \cite{talmor2021commonsenseqa}.
}
\label{tab:results_supervised}
\end{table}

==> [ARR 2021.11] Generated Knowledge Prompting/floats/results_zeroshot.tex <==
\begin{table}[t]
\setlength{\tabcolsep}{4pt}
\footnotesize
\centering
\begin{tabular}{clccc}
\toprule
& \textbf{Inference} & \textbf{Knowledge} & \textbf{dev} & \textbf{test} \\
\midrule
\multirow{4}{*}{\textbf{NS}} & \multirow{2}{*}{T5-11b} & --$^{*}$ & 67.5 & 70.23 | 64.08 \\
& & ours & \textbf{78.0} & \textbf{79.24} | \textbf{72.47} \\
\cmidrule{2-5}
& \multirow{2}{*}{GPT-3} & -- & 72.0 & 74.91 | 66.34 \\
& & ours & \textbf{81.0} & \textbf{80.74} | \textbf{73.46} \\
\midrule
\multirow{2}{*}{\textbf{CSQA}} & \multirow{2}{*}{T5-11b} & -- & 39.89 & -- \\
& & ours & \textbf{47.26} & -- \\
\midrule
\multirow{2}{*}{\textbf{QASC}} & \multirow{2}{*}{T5-11b} & -- & 48.16 & 44.89 \\
& & ours & \textbf{58.32} & \textbf{55.00} \\
\bottomrule
\end{tabular}
\caption{
    Improvement on zero-shot models.
    *: T5-11b baseline on NumerSense \cite{stanford}.
}
\label{tab:results_zeroshot}
\end{table}

==> [ARR 2021.11] Generated Knowledge Prompting/sections/conclusion.tex <==
\section{Conclusion}

% Knowledge Augmentation makes inference models favor desired outputs by (1) increasing the model's expected confidence on desired outputs while decreasing that on undesired outputs, and (2) inducing a variance on the confidence that is larger for desired outputs than for undesired outputs, which can be exploited by the max-ensembling algorithm.\alisainline{might also want to talk about why you focused on commonsense and how the method can potentially be applied for other things too. it's not addressed currently.}
% Weaker input augmentation methods (e.g. Language Augmentation, Context Augmentation) does not have property (1) but still have property (2), thereby can still improve the performance of unsupervised inference models when compared with the baseline.

We introduce generated knowledge prompting, a simple method to elicit and integrate knowledge from language models so as to improve performance on commonsense reasoning tasks.
% Our method is generic, unsupervised, resource-efficient, and engineering-efficient. 
In particular, we generate knowledge statements by prompting a language model with task-specific, human-written, few-shot demonstrations of question-knowledge pairs.
% \hanna{you need a sentence describe the method explaining how it is generic... by using examples.}  
% \hanna{rephrase; again there is a notion of symbolic, etc. }
We show that knowledge can be integrated by simply plugging it in at inference time, with no need to finetune the model for knowledge integration. % with extra knowledge.
% Our method offers a generic approach for incorporating symbolic knowledge into off-the-shelf and fine-tuned language models.
% The unique strength of our approach is...
% It improves any model, whther, without any additional finetuneing in order to learn how to incorporate knowledge.
% Why is it surprising
% plug-and-play
Our method shows effectiveness across multiple datasets, sets the new state-of-the-art on three commonsense reasoning tasks, and works under a variety of settings.
The method's success highlights language models as sources of flexible, high-quality knowledge for commonsense reasoning.
% , domain-specific knowledge, and of massively constructing knowledge bases for arbitrary tasks, which we leave for future work.
% \hanna{Maybe  say something about the future work}
% The improvement brought forth by Generated Knowledge Prompting is aligned with common reasoning procedures.
% And the key ingredients to its success?
% Generate good knowledge, and generate more knowledge.

==> [ARR 2021.11] Generated Knowledge Prompting/sections/experiment.tex <==
\section{Experimental Setup}
\label{sec:experiments}

Here, we describe the implementation details of our method and how they are adapted to each task. 

For knowledge generation, we use GPT-3 \cite{brown2020language} as the underlying language model, where our few-shot prompting method is most effective.
We generate $M=20$ knowledge statements for each question with nucleus sampling $p=0.5$ \cite{holtzman2019curious}, and discard repetitions and empty strings.
Generation is terminated when it exceeds 64 tokens or hits the $\texttt{\textbackslash n}$ token.\footnote{An exception is with the CSQA2 dataset, where for the best results we choose $M=5$ and allow for up to 128 tokens in each generation.}

For inference, we use off-the-shelf T5 \cite{raffel2019exploring} and GPT-3, as well as finetuned models that are state-of-the-art on each dataset, including UnifiedQA (UQA) \cite{khashabi-etal-2020-unifiedqa} and Unicorn \cite{lourie2021unicorn}.
See details in the task setup below.

\subsection{Datasets and Task Setup}

We evaluate our method on four commonsense reasoning datasets which cover a variety of challenges and problem formats.

\vspace{.1cm} \noindent \textbf{NumerSense} \cite{lin-etal-2020-birds} consists of numerical statements about common objects and concepts where for each sentence we need to recover a masked number word.
The choices are integers ranging from zero to ten, plus the word \textit{no}, so the task can be framed as a multiple-choice problem.
Since NumerSense is a diagnostic dataset, we only use zero-shot inference models, which is the current SOTA.
We follow \citet{stanford} who uses the state-of-the-art zero-shot T5 with text-infilling setup and select the choice with highest likelihood on its token(s).
We also implement zero-shot GPT-3 inference, where we plug in each choice to the question and compute the choice probability as the generative probability of the entire sentence, normalized over all the choices.
% \begin{align*}
% $p_I(a|q) = p_{\text{GPT3}}(q\text{.replace}(\text{<mask>}, a))$
% \end{align*}

\vspace{.1cm} \noindent \textbf{CommonsenseQA (CSQA)} \cite{talmor-etal-2019-commonsenseqa} is a 5-way multiple-choice QA dataset about common world scenarios.
We do inference with the zero-shot and finetuned T5 models.
For zero-shot T5, we format the question as text-infilling, and predict the choice with highest sequence-to-sequence language modeling probability.
For finetuned T5 (including UnifiedQA which is SOTA), we use the same setup as \citet{khashabi-etal-2020-unifiedqa}.

\vspace{.1cm} \noindent \textbf{CommonsenseQA 2.0 (CSQA2)} \cite{talmor2021commonsenseqa} is a binary classification dataset where we need to judge whether commonsense statements are true or false.
We only do inference with the finetuned model, due to poor calibration of zero-shot models on this dataset.
We use finetuned Unicorn \cite{lourie2021unicorn}, which is the current SOTA, following the setup in \citet{talmor2021commonsenseqa}.

\vspace{.1cm} \noindent \textbf{QASC} \cite{khot2020qasc} is an 8-way multiple-choice QA dataset about grade school science.
This dataset also includes two pieces of background knowledge per question, whose composition fully answers the question.
We do inference with zero-shot T5 and finetuned T5 (including UnifiedQA which is SOTA), using the same setups as CSQA.

\subsection{Inference Model Setup}

Since all the inference models we use (T5, UnifiedQA, Unicorn) are generative language models, the support to a choice by the inference model is
\begin{align*}
& p_I(a | q) = \frac{\exp s_I(a | q)}{\sum_{a' \in A_q}{\exp s_I(a' | q)}}, \\
& \text{where } s_I(a | q) = \sum_{i=1}^{|a|}{\log{p(a_i | a_{<i}, q)}},
\end{align*}
and $a_i$ is the $i$-th token of choice $a$.

\subsection{Knowledge Generation Baselines}

We study the impact of our knowledge generation method (shorthanded as $K$) by comparing with the following baselines:

\vspace{-.2cm} \paragraph{No knowledge ($\varnothing$)} We refer to inference without any knowledge statements as the \textit{vanilla} baseline.

\vspace{-.2cm} \paragraph{Random sentences ($R$)} Sampling random sentences from the language model without conditioning on the question. We use the same implementation setup as our knowledge generation method (i.e. also using GPT-3, with the same hyperparameters).

\vspace{-.2cm} \paragraph{Context sentences ($C$)} Sampling sentences from the context of the question. This is implemented by sampling text continuations of the question from the language model. We use the same implementation setup as our knowledge generation method.

\vspace{-.2cm} \paragraph{Template-generated knowledge ($T$)} Self-talk \cite{shwartz-etal-2020-unsupervised} uses manually-designed templates to elicit knowledge statements from language models.
For fair comparison, we use GPT-3 as the knowledge generator in self-talk, and bound the number of generations to $M=20$ per question.
Templates and other hyperparameters are kept the same as their original paper.

\vspace{-.2cm} \paragraph{Retrieval-based knowledge ($\mathit{IR}$)} Instead of being generated, knowledge can be retrieved from appropriate sources. We consider the following retrieval-based methods. For NumerSense, knowledge is retrieved from sentences in Wikipedia and GenericsKB. For CSQA2, we use snippets returned by Google when querying the question. For QASC, we use the associated fact sentences that are used to create each question.

\vspace{-.2cm} \paragraph{Answers ($A$)} Instead of generating knowledge, GPT-3 can be prompted to generate direct answers to questions. In the prompts, we use the same input questions as those in knowledge generation, while replacing the knowledge statement with the ground truth answer. We consider two baselines: (1) Generate one answer per question and use this to measure the performance of the few-shot GPT-3 inference model; (2) Generate $M = 20$ answers per question, and use these answers to prompt the SOTA inference models.

% \vspace{.1cm} \noindent \textbf{Gold knowledge ($G$).} This is more like an oracle. In certain datasets, the gold knowledge: a \textit{combined} fact sentence which directly answers the question, and two \textit{separate} fact sentences which, when taking their composition, derive the combined fact sentence. We experiment with using either (1) the \textit{gold combined fact} ($G1$), or (2) the \textit{gold separate facts} ($G2$).

% \hanna{ add template-based and retrieval based }

% \vspace{.1cm}
% For the random sentences and context sentences methods, we sample the same number of statements per question as in our knowledge generation method (i.e. $M=20$). \hanna{Why do we use GPT2large for the baselines, when we use gpt3 for our method? is it a fair comparison?}
% We use GPT2-large \cite{radford2019language} as the generator with nucleus sampling $p=0.9$ and temperature $\tau=0.5$; generation is terminated when hitting a period token.
% For gold knowledge, it is implied that $M=1 \text{ or } 2$.

\section{Experimental Results}

\input{floats/results}

% \hanna{here, add a apragraph showing the roadmap of your results}
% \hanna{shall we report the self talk generation module as the baseline here as well?}
As we will show, our generated knowledge prompting method sets new state-of-the-art results on most datasets we evaluate on, and works well under both zero-shot and finetuned settings.
In particular, our knowledge generation outperforms naive baselines as well as template-based knowledge generation, and is on-par with retrieval-based systems.

\subsection{Overall Performance}

\autoref{tab:results} shows the results on zero-shot and finetuned models following our task setups.

% \input{floats/results_sota}
\vspace{-.2cm} \paragraph{New state-of-the-art.}
% \autoref{tab:results_sota} compares our method with the previous state-of-the-art. \hanna{Not clear if these are fine-tuned or zero shot}
We apply our method on top of the same inference model used in the previous state-of-the-art.
On NumerSense, we achieve a 6\% (66.18 $\rightarrow$ 72.47) improvement over the previous best method based on the zero-shot T5 model.
The previous state-of-the-art among non-retrieval methods on CSQA2 is based on the finetuned Unicorn model, upon which we improve by 2\% (70.2 $\rightarrow$ 73.03).
For QASC, the previous best is based on the finetuned UnifiedQA model, upon which we improve by 3\% (76.74 $\rightarrow$ 80.33).
% We pushed the SOTA among non-IR methods by 2\% on CSQA2 (based on the finetuned Unicorn model) and 3\% on QASC.

% \input{floats/results_zeroshot}
\vspace{-.2cm} \paragraph{Zero-shot settings.} % \hanna{I usually like if paragraphs start with table numbers so we can quickly find where to look.}
Columns $A$, $B_1$, and $D_1$ in \autoref{tab:results} show that our method substantially improves zero-shot inference models, by 7\% to 10\% across NumerSense (64.05 $\rightarrow$ 72.47), CSQA (39.89 $\rightarrow$ 47.26), and QASC (44.89 $\rightarrow$ 55.00).
% We do not evaluate this on CSQA2 due to the poor calibration of zero-shot models on this dataset.

% \input{floats/results_supervised}
\vspace{-.2cm} \paragraph{Finetuned settings.}
Columns $B_2$, $C$, and $D_2$ in \autoref{tab:results} indicate that our method consistently improves upon the vanilla baseline set by finetuned inference models (though by smaller margins than in the zero-shot settings).
% The improvement can be as large as 8\% (UQA-11b on QASC).
% Meanwhile, we note that the gains tend to become smaller when the inference model is directly finetuned on in-domain data (i.e. models with suffix \textbf{-ft}).

\subsection{Knowledge Generation Methods}
\label{sec:quantitative}

% \hanna{This is more interesting, so I moved it up}
% \input{floats/results_qasc_hierarchy}
% \paragraph{Analysis on the quality of knowledge.} \hanna{we need a better title; Our method outperforms other knowledge generation baselines}
% We study the impact of our knowledge generation method compared with different baselines (\hanna{sec..}). %We compare the quality of knowledge from different knowledge generation baselines (\hanna{sec...}) in terms of their effectiveness when used to prompt the inference model.
% \autoref{tab:results_qasc_hierarchy} shows the task performance when each knowledge geneation method is used to prompt the inference model.
\autoref{tab:results} reports the performance with different knowledge generation baselines.
Generally, random sentences barely help and even hurt the inference model, whereas context sentences of the question provide some gain.
In contrast, knowledge generated by our method consistently leads to substantial performance improvements, which implies that our knowledge is of high quality.
% Nevertheless, prompting and integrating the gold knowledge can provide far more improvement to the inference model, indicating that progress can be made by generating even better knowledge.
% \hanna{This first statement is too generic compared to your results; you are only seeing that your; maybe you can say: comparison with retrieval-based }

\vspace{-.2cm} \paragraph{Knowledge is an essential factor.}
The few-shot GPT-3 model is poorly calibrated to directly answer commonsense questions, underperforming our best models by 14\% to 20\% across all tasks.
Even when we use answers generated by few-shot GPT-3 to prompt the SOTA inference models, this still significantly falls behind our method on almost all the tasks and models we consider (with one exception -- CSQA with T5 inference).
Through the medium of \textit{knowledge}, our method can effectively leverage useful information possessed by GPT-3 to help improve even the SOTA models on various commonsense reasoning tasks.

\vspace{-.2cm} \paragraph{Our knowledge outperform template generated knowledge.}
We compare our knowledge generation method with the template-based \textit{self-talk} on the CSQA dev set.
(CSQA is the only task we experiment with that has self-talk templates available.)
%Using the T5-11b inference model, self-talk gets 45.37\%, which is 1.89\% below our method,
Our method leads to a larger improvement over the T5-11b baseline than self-talk (by 1.89\%), showing that it is better at eliciting helpful knowledge from models. % \hanna{maybe better to report the results in a table; you can put the table side-by-side of TAble 9 or Table 8 because they are also narrow. }

\vspace{-.2cm} \paragraph{Our knowledge is comparable with retrieval-based knowledge.}
% One of the top NumerSense submissions retrieves sentences from Wikipedia and GenericsKB, the latter of which is also used to build the NumerSense training set, and prepends these texts to the question.
On NumerSense, the retrieved knowledge only improves inference performance by 0.18\% on test-core and 1.02\% on test-all, while our method further outperforms it by 8.83\% and 7.37\%, respectively.
This shows that knowledge retrieved from a loosely-related knowledge base can be far less useful than our generated knowledge.
% This indicates that knowledge elicited from models can be more helpful for inference than that retrieved from a loosely related knowledge base.
% We also compare our generated knowledge with Google-retrieved knowledge on the CSQA2 task.
On CSQA2, although we are not able to beat the web-retrieved knowledge, our method still bridges the performance gap without referring to Google search.
For QASC, the ``retrieved'' knowledge is actually gold knowledge from a knowledge base that was used to construct the dataset. As a result, our generated knowledge falls significantly short of the retrieved knowledge.
%our generated knowledge is still far below the retrieved knowledge in terms of performance, since the underlying knowledge base for the retrieval was used to build the QASC dataset itself and thus is extremely relevant to the task.
% Overall, while the helpfulness of retrieval-based methods depends on the accessibility of a relevant knowledge base, our method leads to consistent improvement over an inference model without knowledge prompting.
In summary, our generated knowledge is roughly comparable with retrieved knowledge in terms of downstream performance, and is most valuable when there is no appropriate in-domain knowledge base to retrieve from.

\subsection{Analysis}
\label{sec:analysis}

\input{floats/results_qasc_quantity}
\paragraph{Better performance with more knowledge.}
We analyze the impact of the number of generated knowledge statements, $M$, and show the results in \autoref{fig:results_qasc_quantity}. % \hanna{what is M or Km?}
Generally, the performance increases with the quantity of knowledge statements.
It saturates at $M=20$ and begins to decline when more knowledge statements are introduced, which may be because more noisy knowledge is generated. % \hanna{we need an intuition why that is? does it mean that if you generate much and much more it is better? or, there is a stopping point? my guess is.. it would drop because probably at some point you woudl introduce noise?} %, which means another contributor to the success of our method is to generate more knowledge.

\input{floats/results_qasc_ensembling}
\vspace{-.2cm} \paragraph{The knowledge integration method.}
In addition to the knowledge integration method described in \S\ref{sec:method_inference}, we experiment with two alternatives: Mixture-of-Experts (MoE) and Product-of-Experts (PoE) \cite{hinton2002training}.
These make the following modifications to \autoref{eqn:max_ensembling}, respectively:
\begin{align}
\text{MoE: } p_I(a|q,K_q) &\propto \sum_{0 \le m \le M}{p_I(a|q_m)}, \\
\text{PoE: } p_I(a|q,K_q) &\propto \prod_{0 \le m \le M}{p_I(a|q_m)}.
\end{align}
The results in \autoref{tab:results_qasc_ensembling} indicate that our knowledge integration method -- i.e. adaptively choosing the best knowledge to rely on -- is best among the three.

\input{floats/results_numersense_size}
\input{floats/results_numersense_knowledge}
\vspace{-.2cm} \paragraph{Lightweight inference models and amplification.}
We found that the size of inference model affects the magnitude of improvement.
\autoref{fig:results_numersense_size} shows the NumerSense performance gain on top of different sizes of inference model.
As we use smaller inference models, the performance gain increases drastically.
In particular, with our method the smallest T5 model is as powerful as the T5-3b baseline, and T5-large outperforms the GPT-3 baseline.
This indicates that model-generated knowledge can enable high performing, yet lightweight, inference models.
% that our method brings huge advantage to less powerful inference models.
Furthermore, the improvement does not diminish as the inference model becomes as big as the knowledge generation model, as the inference by GPT-3 can benefit by 9.0\% from the knowledge elicited from itself.
This indicates that our method can somewhat \textit{amplify} the useful knowledge already possessed by the model, leading to better predictions.

\vspace{-.2cm} \paragraph{The size of knowledge generation model.}
\autoref{fig:results_numersense_knowledge} shows the NumerSense performance gain when using different sizes of GPT-3 as the knowledge generation model.
On top of the T5-11b inference model, The 6.7B knowledge model gives a 5.0\% improvement, narrower than the 10.5\% improvement given by the 175B knowledge model.
The 1.3B and 0.4B knowledge models do not give a significant improvement.
Therefore, we do not necessarily need the largest version of GPT-3 as the knowledge source, though we do need the model to be relatively large in order to generate useful and reliable knowledge.

\subsection{Human Evaluation}
\label{sec:human}

\input{floats/human}

We conduct a human evaluation on NumerSense and QASC to study the quality of generated knowledge and the interpretability of its impact on task performance. % We use the NumerSense and QASC datasets. %Through human evaluation, we show that our generated knowledge has high quality and usually impacts model predictions in a human interpretable way.

\vspace{-.2cm} \paragraph{Evaluation.} We report the quality of knowledge statements along four axes: (1) \textit{Grammaticality}: whether it is grammatical; (2) \textit{Relevance}: whether it is relevant to the topic or concepts mentioned on the question; (3) \textit{Factuality}: whether it is (mostly) factually correct; and (4) \textit{Helpfulness}: whether it helps answering the question in an either direct or indirect way, and may fall into one of the three categories: helpful (i.e. supports the correct answer), harmful (i.e. negates the correct answer or supports an incorrect answer), or neutral (neither helpful nor harmful).
These metrics are adapted from \citet{shwartz-etal-2020-unsupervised} and are defined in Appendix \ref{sec:guidelines}.

From each dataset, we sample up to 50 \textit{selected knowledge} (\S\ref{sec:method_inference}) that change the correctness of T5-11b's prediction (i.e. rectifies model prediction from wrong to right, or misleads model prediction from right to wrong).
The knowledge are labeled by two NLP experts and a moderate level of agreement was reached (Fleiss Kappa $\kappa = 0.57$ \cite{landis1977measurement}).
To ensure objectivity, it is not revealed to the annotators whether the knowledge rectifies or misleads the model prediction.

\vspace{-.2cm}  \paragraph{Results.} \autoref{fig:human} summarizes the results.
The vast majority of selected knowledge are grammatical and relevant to the question, and 83\% of them are factually correct.
72\% are seen as being helpful for answering the question according the human evaluators, whereas 13\% are harmful.
% There is also a good agreement between human and machine's perception on whether knowledge is helpful or harmful.
Out of the knowledge statements that rectify the model predictions, 93\% are labeled as helpful by the human evaluators; in contrast, when the knowledge statement misleads the model, only 21\% are labeled as helpful, and 39\% harmful.
% are in  are and in particular human can see why a knowledge statement rectifies the model prediction 93\% of the time.
Of the knowledge deemed helpful by human \textit{and} rectifies model prediction, 95\% are factual, while of those deemed harmful by human \textit{and} misleads model prediction, 86\% are non-factual, suggesting that improving knowledge factuality is a promising path towards more helpful knowledge.
%
We also analyzed the non-selected knowledge and found that these statements have slightly lower factuality and helpfulness than the selected knowledge.
% This shows that our knowledge integration method does well at selecting high-quality knowledge.

\subsection{Qualitative Examples}
\label{sec:qualitative}

\input{floats/qualitative}

\autoref{tab:qualitative} shows a few examples where the generated knowledge rectifies model prediction.
Due to space constraints we only show the \textit{selected knowledge} (\S\ref{sec:method_inference}) for each question.
In all examples, the model without prompted knowledge assigns a higher score to an incorrect answer than the correct answer, while with knowledge prompting, the correct answer is assigned a much higher score. % and beats the distractor.
Prompting with generated knowledge can transform commonsense reasoning into explicit reasoning procedures such as paraphrasing, induction, deduction, analogy, abductive reasoning, logical elimination, negation, and numerical reasoning.

==> [ARR 2021.11] Generated Knowledge Prompting/sections/introduction2.tex <==
\section{Introduction}
\label{sec:introduction}

\input{floats/diagram}
\input{floats/examples}

Commonsense reasoning tasks involve selecting or generating plausible inferences about everyday scenarios \cite{sap-etal-2020-commonsense}.
% Performing commonsense reasoning requires commonsense knowledge.
While pretrained language models implicitly contain a large amount of knowledge and can be directly used for commonsense reasoning \cite{trinh2018simple, yang-etal-2020-designing}, incorporating external knowledge bases (such as ConceptNet \cite{speer2017conceptnet} and ATOMIC \cite{sap2019atomic}) can boost performance on some of these tasks \cite{mitra2019additional, bian2021benchmarking}. 
On the other hand, language models themselves can serve the role as knowledge bases, as they allow for querying knowledge by completing natural language statements \cite{petroni-etal-2019-language, jiang-etal-2020-know}.
To leverage knowledge contained in language models for answering commonsense questions, most recent work manually designs dataset-specific, cloze-style templates to generate certain types of \textit{knowledge statements} (i.e. knowledge expressed as natural language statements), such as clarifications \cite{shwartz-etal-2020-unsupervised} or contrastive explanations \cite{paranjape-etal-2021-prompting}.
% , then conditions on the statements during prediction.
% integrates the knowledge into the inference process.
However, tasks often require different types of knowledge that are beyond the scope of pre-defined templates (\autoref{tab:examples}).
% , and the effect of the mechanism for integrating the knowledge remains unclear.

In this paper, we develop a simple, yet effective, method for eliciting useful knowledge statements from language models and using the knowledge to improve prediction performance. % \hanna{revise the last sentence; similar as the abstract, mention  you generate this knowledge with prompting and demonstration} -- It is mentioned in a later sentence of this paragraph. By the way, I feel that the introduction could be more high-level and we don't necessarily need to give too much details? 
Our method (sketched in \autoref{fig:diagram}, called  \textit{generated knowledge prompting}) consists of two steps%. % uses two language models sequentially: a \textit{knowledge model} and an \textit{inference model}. % \hanna{the phrase our method is kind of overloaded; generated knowledge prompting is the knwoledge model, or the full pipeline?} -- This should be resolved in the current draft, "our method" is the full pipeline; If we need to refer to the knowledge generation only, I would say "our knowledge generation method".
: (1) generating question-related knowledge statements from a language model by conditioning on human-written demonstrations, and (2) using a language model to make predictions with each knowledge statement, then selecting the highest-probability prediction.
% First, we generate question-related knowledge statements from a language model by conditioning on a prompt that contains instructions and few-shot demonstrations. %, which are question-knowledge mappings \hanna{what is question-knowledge mapping? Instead, be more explicit; these demonstrations  are... written by humans for a few examples in each task. Here yo ushould mention that those demonstrations are fixed for each task, and then you are using it for every instance  } written by human.
% These human-written demonstrations show typical questions and helpful knowledge statements for the given task.
% A second language model then uses the generated statements to make a prediction.
% Each knowledge statement is passed to a second language model, which makes a prediction 
% Then we use a second language model to make predictions with each knowledge statement, and select the highest-probability prediction.
% Then, the generated knowledge are integrated into the decision process, where we prompt an inference model with knowledge statements and select the knowledge that maximizes prediction probability.

Experiments show that our method improves both zero-shot and finetuned models on numerical commonsense (NumerSense \cite{lin-etal-2020-birds}), general commonsense (CommonsenseQA 2.0 \cite{talmor2021commonsenseqa}), and scientific commonsense (QASC \cite{khot2020qasc}) benchmarks. % \hanna{cite datasets}
% We take pretrained language models off-the-shelf, use prompts and demonstrations to elicit knowledge statements that transform the commonsense question answering into an explicit reasoning procedure, and prompt the inference model with such knowledge.
% An integration algorithm can adaptively select the best knowledge to inform the decision of inference model.
% This process is unsupervised and resource-efficient, since we do not need a training set to finetune the knowledge generation or inference model, or an in-domain knowledge base to retrieve knowledge from.
% It is also more generic and engineering-efficient compared to previous methods, making it easily adaptable to various tasks.
% 
% We apply our method on recent commonsense reasoning datasets -- NumerSense, CommonsenseQA, CommonsenseQA 2.0, and QASC -- and demonstrate that we can push the limits of existing models.
% Our method improves the state-of-the-art of NumerSense by about 9\%, that of CommonsenseQA 2.0 by about 2\%, and that of QASC by about 3\%.
It shows superior performance over the template-based knowledge generation approach \textit{self-talk} \cite{shwartz-etal-2020-unsupervised}, and 
performs comparably to
% is comparable to and even outperforms 
retrieval-based systems.
% Experimental results show the effectiveness of our method under a variety of settings: with different sizes of inference models, and with both zero-shot and finetuned inference models.
% Notably, it is effective when knowledge generation and inference are done with the same language model.

Our analysis show that three factors contribute to the performance of the generated knowledge prompting method: (i) the \textit{quality} of knowledge -- e.g. our generated knowledge outperforms template-based systems, (ii) the \textit{quantity} of knowledge -- i.e. performance improves with more knowledge statements, and (iii) the strategy for integrating knowledge during inference.
% 
% We identify three factors that contribute to its performance improvements: the high quality of generated knowledge, the large quantity of the knowledge, and the clever selection of good knowledge for inference.
Qualitative analysis suggests that our generated knowledge are of generic types % \hanna{what do you mean by generic types?} -- We defined generic types before, it's one of the desired properties of knowledge and a partial motivation of our method, so I thought we should mention it here.
and can reduce commonsense question answering to explicit reasoning procedures -- e.g. deduction -- that are supported by off-the-shelf and finetuned language models.
% Our work provides a simple recipe for using language models as sources of symbolic knowledge in prediction tasks, and highlights the influence of symbolic knowledge in neural reasoning.
% , and , and we hope that the insights we share will inspire further efforts on neuro-symbolic knowledge integration.

==> [ARR 2021.11] Generated Knowledge Prompting/sections/introduction3.tex <==
\section{Introduction}
\label{sec:introduction}

\input{floats/diagram}
\input{floats/examples}

It remains an open research question whether external knowledge is needed for commonsense reasoning. On one hand, a substantial body of prior work has reported that integrating external knowledge can help improve task performance \cite[\textit{inter alia}]{mitra2019additional, bian2021benchmarking}, especially if the knowledge is high quality (e.g. hand-crafted by experts). On the other hand, recent leaderboards are often dominated by large-scale pretrained models that are fine-tuned on a target benchmark \cite{khashabi-etal-2020-unifiedqa, lourie2021unicorn}, suggesting that the benefits of external knowledge may wash away as the underlying models increase in size and are pretrained on ever larger amounts of raw text. 

Even if external knowledge is found to be effective on a particular task, \textit{flexibility} remains a fundamental hurdle to integrating external knowledge,
% Upon a closer look, 
% while there are empirical evidences that task-specific knowledge can indeed be helpful, especially if the knowledge is high quality (e.g., hand-crafted by experts),  
% there are several fundamental challenges to robustly integrating external knowledge for commonsense reasoning. 
as many benchmarks currently lack appropriate knowledge bases with sufficient coverage. Furthermore, prior methods often require task-specific, custom supervision for knowledge integration \cite{mitra2019additional, chang-etal-2020-incorporating}, introducing a burden for rapidly adapting new pretrained models to a wide variety of tasks.

In this paper, we investigate whether external knowledge can be helpful for commonsense reasoning, even on top of the largest state-of-the-art pretrained models (e.g. T5-11b \cite{raffel2019exploring} and its variants), with a focus on four recent commonsense benchmarks.
% that are not yet supported by existing commonsense knowledge bases. 
To facilitate easier adaptation with any zero-shot or finetuned models, we propose an approach that does not require access to a structured knowledge base or joint finetuning for knowledge integration.

The key insight behind our method, Generated Knowledge Prompting (sketched in \autoref{fig:diagram}), is that we can generate useful knowledge from a language model, then provide the knowledge as an input prompt that is concatenated with a question.
% , without any custom fine-tuning. 
% Our method does not require fine-tuning or access to a structured knowledge base, 
% % the resulting models are not fine-tuned to incorporate the provided knowledge, 
% yet it boosts performance considerably, even improving state-of-the-art models on three hard commonsense reasoning benchmarks. 
%
%There has been an alternating pattern on the commonsense reasoning leaderboards: at some point a method that incorporates external knowledge bases to the existing best model sets new state-of-the-art, and later it is outcompeted by a larger model that does not use extra knowledge, and the cycle repeats.
%On one hand, this is a clear indication that task-related knowledge is helpful to model performance, while the appropriate knowledge base is not always readily available for every task.
%On the other hand, incorporating extra knowledge often requires dedicated submodules or further finetuning \cite{mitra2019additional, chang-etal-2020-incorporating} so that the model can work with the extra knowledge, which sets barriers for new base models to adopt explicit knowledge.
To support a variety of settings without finetuning, the quality and flexibility of knowledge is crucial. We propose a simple, yet effective, method that elicits \textit{knowledge statements} (i.e. knowledge expressed as natural language statements) from generic language models in a few-shot setting. Compared to prior work that elicits knowledge via clarification questions \cite{shwartz-etal-2020-unsupervised} or contrastive explanations \cite{paranjape-etal-2021-prompting}, our approach can generate knowledge flexibly, beyond the scope of pre-defined templates (\autoref{tab:examples}). 
%We provide a comprehensive empirical study to compare alternative means to acquire knowledge.

%More concretely, our method, \textit{generated knowledge prompting}), consists of two steps: (1) generating question-related knowledge statements from a language model by conditioning on task-specific, human-written, few-shot demonstrations, and (2) using a language model to make predictions with each knowledge statement, then selecting the highest-probability prediction.
%To generate knowledge from models, some recent work manually designs dataset-specific, cloze-style templates to generate certain types of knowledge such as clarifications \cite{shwartz-etal-2020-unsupervised} or contrastive explanations \cite{paranjape-etal-2021-prompting}, whereas our method can flexibly generate knowledge statements of generic types that are beyond the scope of pre-defined templates (\autoref{tab:examples}).

Experiments show that our method improves both zero-shot and finetuned models on numerical commonsense (NumerSense \cite{lin-etal-2020-birds}), general commonsense (CommonsenseQA \cite{talmor-etal-2019-commonsenseqa}, CommonsenseQA 2.0 \cite{talmor2021commonsenseqa}), and scientific commonsense (QASC \cite{khot2020qasc}) benchmarks, setting a new state-of-the-art on three of these datasets.
It outperforms the template-based knowledge generation method \textit{self-talk} \cite{shwartz-etal-2020-unsupervised}, while performing comparably to retrieval-based systems.

We find three factors contribute to the performance of generated knowledge prompting: (i) the \textit{quality} of knowledge, (ii) the \textit{quantity} of knowledge where the performance improves with more knowledge statements, and (iii) the strategy for integrating knowledge during inference. 
Our qualitative analysis suggests that the generated knowledge statements cover a variety of types, and can transform commonsense question answering to explicit reasoning procedures, e.g. deduction, that are supported by off-the-shelf and finetuned language models.


==> [ARR 2021.11] Generated Knowledge Prompting/sections/method.tex <==
\section{Generated Knowledge Prompting}
\label{sec:method}

\input{floats/prompt}

A multiple-choice commonsense reasoning task involves predicting an answer $a\in A_q$ given a question $q\in Q$, where the set of choices $A_q$ is finite and can vary by question, and both questions and answers are variable-length text sequences.
Our method answers commonsense questions in two steps.

The first step is \textit{knowledge generation}, where we use a language model $p_G(k|q)$ to generate knowledge statements conditioned on the question:
\begin{align*}
K_q &= \{ k_m : k_m \sim p_G(k|q), m = 1 \ldots M \},
\end{align*}
where each knowledge statement $k_m$ is a variable-length text sequence.
Intuitively, each statement contains information that is helpful for answering the question (e.g. \autoref{tab:examples}).

The second step is \textit{knowledge integration}, where generated knowledge is integrated into the decision process of a language model used for inference,
\begin{align*}
\hat{a} &= \argmax_{a \in A_q}{p_I(a|q,K_q)}.
\end{align*}
In contrast, the \textit{vanilla} setting of using the inference model without knowledge is represented by $\hat{a} = \argmax_{a \in A_q}{p_I(a|q)}$.
% Generated knowledge prompting is an extension of using the inference model without knowledge (i.e. the \textit{vanilla} setting), 
% Let $P_i(a\mid q,K_q)$ denote an aggregate inference model which produces a score for answer choice $a$ by additionally taking the knowledge set $K_q$ as input. Then, the final answer choice is given by
% \begin{align*}
% \hat{a} &= \argmax_{a \in A_q}{P_I(a|q,K_q)}
% \end{align*}

% Then, use these knowledge statements to prompt the inference model:
% \begin{align*}
% \hat{a} &= \argmax_{a \in A_q}{P_I(a|q,K_q)}
% \end{align*}
% where $P_I(a|q,K_q)$ is the aggregated choice score over the knowledge set $K_q$, as defined by a knowledge integration algorithm.

% Here, we describe  the knowledge model (Section~\ref{sec:method_generation}) to generate high-quality, flexible knowledge, and the inference model (Section~\ref{sec:method_inference}) to integrate knowledge and predict the final answer. 
% Next, we describe the knowledge models that we use to generate high-quality, flexible knowledge, and the inference model that we use to integrate knowledge into prediction.
% Below we describe the our knowledge generation and integration methods.
Next, we describe the knowledge generation and integration steps in detail.

\subsection{Knowledge Generation}
\label{sec:method_generation}

We generate question-related knowledge statements by prompting a language model.
The prompt consists of an instruction, a few demonstrations that are fixed for each task, and a new-question placeholder.
The demonstrations are human-written, and each consists of a question in the style of the task and a knowledge statement that is helpful for answering this question.
%
For a given task, we write five demonstrations using the format in \autoref{tab:prompt}.
%
% \sean{highlight that the generic format is the same for all tasks (instruction $i$, demonstrations $(q,k)_j$)}
% We generate knowledge statements by prompting language models with demonstrations of useful question-related knowledge. \hanna{task related?} \hanna{I would write like this: The prompt consists of an instruction and a few examples that are fixed for each task; then explain how the examples are collected. then move on to the following.}
% The prompt uses the same generic format across all tasks. %
% It consists of an instruction sentence, a few demonstrations of question-knowledge pairs, and ends with a question placeholder (\autoref{tab:prompt}). \hanna{This paragraph seems that you are providing examples for every instance, whereas you are doing it for some examples in each task.}
%
% \hanna{I would move this sentence right after the first sentence to mention that demonstrations are fixed for a given task. }For a given task, we gather five questions resembling those in the task, and write a corresponding knowledge statement for each question.
% \hanna{then start describing the criteria for your demonstrations; The desiderata for  knowledge statements used for demonstrations is ... the goal of the statements is to show LMs the human reasoning behavior, therefore these knowledge statements are collected .... } 
% Here are some guidelines for writing the demonstrations.

We write questions (or select them from the training set, when available) that are representative of challenges posed by the task (e.g. numerical commonsense, scientific commonsense).
% , or select and may be selected from the training set if one is available.
% They may be creatively written by human, or chosen from a small subset of the training set for the task if one is available.
We pair each question with a knowledge statement that turns the commonsense problem posed by the question into an explicit reasoning procedure, without directly answering the question.
% Meanwhile, it should not be the simple declarative statement that combines the question and answer, so as to encourage more diverse generations.
For example, the knowledge statement \textit{\uline{Birds have two wings. Penguin is a kind of bird.}} is helpful for the question \textbf{\uline{Penguins have <mask> wings}}, because it turns the problem into deductive reasoning.
% , a good knowledge statement would be: 
% The two sentences in the knowledge statement can be viewed as a complete set of premises for deductive reasoning.
Meanwhile, \textit{\uline{Penguins have two wings.}} would be a poor knowledge statement to demonstrate according to our guideline.

% We create five question-knowledge pairs for each dataset and format them as demonstrations as shown in \autoref{tab:prompt}.
% The prompt for knowledge generation starts with an instruction sentence, followed by the demonstrations, and ends with a question placeholder.
When generating knowledge for a new question $q$, we plug the question into the placeholder, and repeatedly sample generated continuations of this prompt to obtain a set of knowledge statements $K_q = \{ k_1, k_2, \hdots, k_M \}$.
% The prompt is fixed when generating knowledge for questions from the same dataset.
For full prompts on all the tasks we evaluate on, see Appendix \ref{sec:prompts}. % \hanna{In this paragraph bring back some of your notations that you introduced earlier; when generating knowledge for a particular question q that; a set of knowledge statements Kq} \hanna{what do you mean by sampling? }

% We present two unsupervised knowledge generation methods, one based on example-based prompting and the other utilizing a constrained decoding algorithm.
% In both methods, for each question we repeatedly sample the generation for $M$ times to get a diverse set of knowledge statements.

% \paragraph{Example-based prompting.}
% We elicit knowledge from very powerful pretrained language models, like GPT3 \cite{brown2020language}, by designing a prompt and handcrafting a few example generations for each dataset.
% For instance, \autoref{tab:prompt_numersense} shows our prompt for NumerSense. \hanna{Here, refer to an appendix or a table that shows the list of prompts for different datasets. }

% \paragraph{Constrained decoding.}
% Since there may be limited access to models that are large enough to do well at in-context learning, we also propose a knowledge generation method that is based on constrained decoding \cite{lin-etal-2020-commongen}.
% % Our knowledge generation method is inspired by the CommonGen task, where the model needs to generate a plausible sentence that includes a given set of words.
% We extract salient words or phrases from the question, and ask models to generate knowledge-like sentences that contain these \textit{seed texts}. \hanna{why seed texts and why not salient words? how do you define salient words.}
% For each task, seed texts are extracted with a customized method. \hanna{this sentence is vague}
% For example, for NumerSense the seed texts are noun tokens from the question using the FLAIR part-of-speech tagger.  \hanna{same here; refer to a table or appendix for details on other datasets.}
% We use NeuroLogic \cite{lu-etal-2021-neurologic} as the constrained decoding algorithm and run it on top of GPT2 \cite{radford2019language}.

\subsection{Knowledge Integration via Prompting} % \hanna{Rename to Inference Model}
\label{sec:method_inference}
In the knowledge integration step, we use a language model -- called the inference model -- to make predictions with each generated knowledge statement, then select the highest-confidence prediction.
% Suppose we have an inference model $p_I(a|q)$ that answers questions in a certain task.
% In the knowledge integration step, we additionally prompt the inference model with the knowledge generated in the previous step.
% Suppose for each question $q$ we generated $M$ knowledge statements: $K_q = \{ k_1, k_2, \hdots, k_M \}$. \hanna{This statement should be moved to the previous section.}
% \hanna{Mostly try to write like this: The inference model selects   the answer a among possible choices .... by prompting a langauge model  with a given the question q and the generated knowledge statements K.}
% We will \textit{prompt} the inference model with the knowledge. \hanna{Here, I am confused; what is your inference model? is your inference model the whole setup of prompting langauge models with knowledge and q, or just the language model?}
Specifically, we use each knowledge statement to prompt the model, forming $M$ knowledge-augmented questions:
\begin{align*}
q_0 = q, q_1 = [k_1 || q], \hdots, q_M = [k_M || q],
\end{align*}
where $[\cdot || \cdot]$ denotes text concatenation.

We compute an aggregated score for each answer choice $a$ using the augmented question that best supports it under the inference model: % \hanna{rather than writing it as "we define" say the model computes the an aggregated score for each chocie a using... }
\begin{align}
p_I(a|q,K_q) &\propto \max_{0 \le m \le M}{p_I(a|q_m)}. \label{eqn:max_ensembling}
\end{align}
Intuitively, this favors knowledge statements that strongly support one of the choices.
% while filtering out those that fail to let the inference model make a resolute decision.

The predicted answer is then,
\begin{align*}
\hat{a} &= \argmax_{a \in A_q}{\max_{0 \le m \le M}{p_I(a|q_m)}},
\end{align*}
which is the choice that gets most support from one of the knowledge statements.
This prediction uses a single knowledge statement, which we refer to as the \textit{selected knowledge}: 
\begin{align*}
\hat{k} &= k_{\hat{m}} \text{ where } \hat{m} = \argmax_{0 \le m \le M}{\max_{a \in A_q}{p_I(a|q_m)}}.
\end{align*}

The inference model may be any existing language model taken off-the-shelf (i.e. zero-shot) or finetuned on the task.
We do not do any further finetuning with knowledge prompting.

==> [ARR 2021.11] Generated Knowledge Prompting/sections/related_work.tex <==
\section{Related Work}

\paragraph{Knowledge can be elicited from pretrained language models.}
Numerous works have shown that pretrained language models implicitly contain a large amount of knowledge that can be queried via conditional generation \cite{davison-etal-2019-commonsense, petroni-etal-2019-language, jiang-etal-2020-know}.
Consequently, these models can directly perform inference on tasks like commonsense reasoning \cite{trinh2018simple, yang-etal-2020-designing}, text classification \cite{shin-etal-2020-autoprompt, puri2019zero}, and natural language inference \cite{shin-etal-2020-autoprompt, schick-schutze-2021-exploiting}.
% (CohRank - Winograd, CommS2S - WinoGrande|OpenBookQA|ARC)
% (AutoPrompt - sentiment analysis)
% (AutoPrompt)
Inspired by these observations, we elicit question-related knowledge in an explicit form from language models and use them to guide the inference.
% TODO: cite AutoTOMIC and GenGen
% be used to construct/expand/complete commonsense knowledge bases (LMComm, AutoTOMIC, GenGen) or 

\vspace{-.2cm} \paragraph{Leveraging external knowledge for commonsense reasoning.}
Some work uses external commonsense knowledge bases to make improvements on various NLP tasks, including commonsense reasoning.
One approach is to inject commonsense knowledge into language models, either by pretraining on knowledge bases \cite{ma2021knowledge, chang-etal-2020-incorporating, mitra2019additional, zhong2019improving} or finetuning the model so that it can reason with additional retrieved knowledge \cite{chang-etal-2020-incorporating, mitra2019additional, bian2021benchmarking}.
Another direction is to ground the question into a knowledge graph and do inference with graph-based reasoning \cite{lin-etal-2019-kagnet, lv2020graph, yasunaga-etal-2021-qa}.

A common prerequisite of these methods is a high-quality, high-coverage, in-domain commonsense knowledge base \cite{ma-etal-2019-towards}.
% It has been shown that, in order for the knowledge to be effective, it is important to use a KB with high domain overlap with the dataset \cite{ma-etal-2019-towards}.
Some commonsense reasoning datasets are derived from existing knowledge bases; for example, CommonsenseQA \cite{talmor-etal-2019-commonsenseqa} is derived from ConceptNet \cite{speer2017conceptnet}, and Social IQA \cite{sap-etal-2019-social} is derived from ATOMIC \cite{sap2019atomic}. %, and $\alpha$NLI \cite{bhagavatula2019abductive} is derived from ROC-Stories \cite{mostafazadeh-etal-2016-corpus}.
For such datasets, it is natural to elicit related knowledge from the underlying knowledge base that derived them, and typically this would demonstrate considerable gains \cite{mitra2019additional, chang-etal-2020-incorporating}.
However, if there is a domain mismatch between the dataset and the knowledge base, such gains tend to diminish \cite{mitra2019additional, ma-etal-2019-towards}.
This becomes a bottleneck when encountering datasets that have no suitable knowledge base (e.g. NumerSense \cite{lin-etal-2020-birds} and CommonsenseQA 2.0 \cite{talmor2021commonsenseqa}), or when the system needs to handle commonsense queries that do not fit in any of the commonsense domains represented by an existing knowledge base.
Our work overcomes this difficulty by leveraging  pretrained language models as the source of commonsense knowledge.

\vspace{-.2cm} \paragraph{Adding generated text during inference.}
Recently, several works show that model performance on commonsense reasoning can be boosted by augmenting the question with model-generated text, such as clarifications, explanations, and implications.
Self-talk \cite{shwartz-etal-2020-unsupervised} elicits clarifications to concepts in the question and appends them to the inference model input.
% This method designs task-specific templates used for inquiring the model, which is only capable of eliciting a limited variety of knowledge and requires expert engineering when transferring to new tasks.
% In addition, Self-Talk needs to query the generator twice -- once for generating the clarification questions to ask and another for generating answers to a given question.
% This results in quadratic number of candidate clarifications and significantly slows down inference.
Contrastive explanations \cite{paranjape-etal-2021-prompting} prompts inference models with generated explanations that contrast between two answer choices.
% The explanation generation is also based on a set of templates that is heuristically obtained from the datasets and is not shown to generalize to new tasks.
The aforementioned methods depend on task-specific templates to inquire the generator, which means they are only capable of eliciting a limited variety of knowledge and require careful hand-crafting to transfer to new tasks.
% This method is designed for 2-way multiple-choice tasks, and its complexity would grow quadratically w.r.t. the number of choices.
% Moreover, the answer choices must be known to the generator model \textit{a priori}, meaning that it cannot be easily adapted to generative commonsense tasks.
Other explanation-based methods \cite{latcinnik2020explaining, rajani-etal-2019-explain} finetune the generator model so that it produces explanations that are used for question augmentation.
DynaGen \cite{bosselut2021dynamic} uses pretrained commonsense models to generate implications of a question and builds a dynamic graph of natural language statements on which reasoning is conducted.
However, its usage of COMeT \cite{bosselut-etal-2019-comet} as the generator confines its applicability to the social commonsense domain.
Our work contributes to this general line of research, yet different from these previous methods that elicit knowledge with task-specific templates or from finetuned knowledge generators, 
% often make task-specific assumptions on the type of knowledge to generate, 
our method requires only a few human-written demonstrations in the style of the task, making it much more flexible, easy-to-transfer, and engineering-efficient.
% something like this? idk feel free to rewrite obv
%approach this from a reasoning perspective and aim to generate arbitrary knowledge that can support an explicit reasoning procedure, % take an approach that generates knowledge truly needed by the model to perform sound reasoning. \yejin{"truly needed" "sound reasoning" --- both are a tad much...}
%making our method flexible, easy-to-transfer, and engineering-efficient.

==> atrash/analysis.tex <==
\section{Good Knowledge, and More Knowledge}
\label{sec:analysis}

\input{floats/qasc_summary}

Why Generated Knowledge Prompting works, after all?
Through the following quantitative study of the behavior of the inference model, we show that the performance boost is due to two factors: the quality of knowledge, and the max-ensembling algorithm on a diverse set of knowledge.
% We hope to provide more insight by quantitatively characterizing the behavior of the inference model under \name{}.
We choose to study the QASC dataset in particular because it comes with annotated ground knowledge, and we will focus on two metrics of the inference model: the mean and variance of the answer scores.

\textbf{Metrics.}
For each question, we generate multiple knowledge sentences.
An answer choice may be evaluated differently by the inference model when prompted with each knowledge sentence, thus inducing a list of scores: $\{ p_I(a \mid [k_m||q]) \}$.
We define \textit{induced average} and \textit{induced deviation} as the mean and standard deviation of these scores, and denote them as $\mu_K(q,a)$ and $\sigma_K(q,a)$, respectively.
Because eventually predictions are made based on only one of the prompts (selected by the max-ensembling algorithm), we also define the \textit{selected score} as the score of an answer under the selected prompt:
\begin{align*}
\omega_K(q,a) &= p_I(a \mid [\hat{k}||q])
\end{align*}
where $\hat{k} = \argmax_{k \in K_q}{\max_{a \in A_q}{p_I(a \mid [k||q])}}$.
For the vanilla inference method (i.e with no knowledge prompting), we define
\begin{align*}
\mu_\varnothing(q,a) = \omega_\varnothing(q,a) = p_I(a|q), \sigma_\varnothing(q,a) = 0
\end{align*}
Since we are interested in the general trend due to our method, we compute the mean of these metrics over the entire dataset, while making a particular distinction between correct answers and distractors:
\begin{align*}
\bar{X}^* &= \text{Mean}_{(q,a^*) \in D}[X(q,a^*)] \\
\bar{X}' &= \text{Mean}_{(q,a^*) \in D, a' \in A_q \backslash \{a^*\}}[X(q,a')]
\end{align*}
where $X \in \{ \mu, \sigma, \omega \}$.
Note that $\bar{\mu}^*$ can be viewed as a continuous proxy to the prediction accuracy under the Mixture-of-Experts ensembling algorithm (\autoref{eqn:moe}).

\textbf{Baselines.}
We consider a few alternatives to \textit{ground knowledge} as the prompt:


\textbf{Discussion.}
\autoref{fig:qasc_summary} plots the aforementioned metrics of a T5-11b inference model on the QASC dev set.

Looking at the mean of average score (the dashed lines), we conclude that
\begin{align*}
\bar{\mu}_\varnothing^* \approx \bar{\mu}_L^* &\approx \bar{\mu}_C^* < \bar{\mu}_K^* \\
\bar{\mu}_\varnothing' \approx \bar{\mu}_L' &\approx \bar{\mu}_C' > \bar{\mu}_K'
\end{align*}
This tells us that on average, prompting with the generated knowledge increases the scores for correct answers and decreases the scores for distractors, thereby improving the prediction accuracy.
In comparison, language prompting ($L$) and context prompting ($C$) do not move this metric significantly, while prompting with gold facts ($G2$ and $G1$) show similar trend as Generated Knowledge Prompting, yet with larger magnitude.
This indicates that the generated knowledge are generally effective, while with inferior quality than the gold annotated knowledge.
The better knowledge we have, the more we can help the inference model.

Next, the error bars and the mean of selected score (solid lines) show that
\begin{align*}
\bar{\sigma}_i^* > \bar{\sigma}_i' &\text{ for } i \in \{ K, C, L \} \\
\bar{\omega}_\varnothing^* \approx \bar{\omega}_L^* &< \bar{\omega}_C^* << \bar{\omega}_K^* \\
\bar{\omega}_\varnothing' \approx \bar{\omega}_L' &> \bar{\omega}_C' >> \bar{\omega}_K'
\end{align*}
(Note that the score axis uses a logistic scale, so the standard deviation is not intuitive to see.)
This tells us that the induced variance of the scores tend to be larger for correct answers than for distractors.
Since extreme scores help knowledge and answers stand out in the max-ensembling algorithm, the larger induced variance further helps correct answers to beat the distractors.
Note that this observation is also true for language prompting ($L$) and context prompting ($C$).
The combined effect of induced average and induced deviation results in an amplified boost as shown by the selected scores $\bar{\omega}$.
Having good knowledge and more knowledge are therefore both indispensable ingredients to the success of our method.

==> atrash/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Performing commonsense reasoning requires commonsense knowledge.
Although pretrained language models implicitly contain a large amount of knowledge and can be directly applied for commonsense reasoning \cite{trinh2018simple, yang-etal-2020-designing}, incorporating external knowledge bases can boost performance on some of these tasks \cite{mitra2019additional, bian2021benchmarking}. % \yejin{This statement comes across as inaccurate over-claim... "usually" is too strong as it sounds like "almost always". more accurate phrasing would be "can boost ... on some of these tasks"} 
On the other hand, language models themselves can serve the role of knowledge bases as they allow for querying \textit{symbolic knowledge} (i.e. knowledge expressed as natural language statements) via conditional generation \cite{petroni-etal-2019-language, jiang-etal-2020-know}.
% \yejin{this sentence is not entirely accurate. the prior work was trying to be catchy with their titles, which we took too literally here. also, when we use the word "mine", it already implies that the source is not a KB, just raw noisy stuff mixed with other stuff... a more accurate phrasing would be "On the other hand, PLMs themselves can serve the role of knowledge bases as they allow for querying symbolic knowledge via conditional generation"}
Therefore, we explore the following question: Can we use statements of knowledge elicited from language models to improve model performance on commonsense reasoning tasks?

\input{floats/diagram}
\input{floats/qualitative}

% With the recent boom of prompt-based learning, it is widely known that a large variety of knowledge can be elicited from PLMs \cite{}.
% Also intensively studied is that incorporating external knowledge can improve the performance of LM-based inference on various tasks, including CSR \cite{}.
% Therefore, a natural research question to ask is: Are knowledge elicited from LMs themselves helpful for the LMs' inference?

We observe that model predictions on commonsense questions can be rectified when prompted with simple but relevant knowledge statements.
\autoref{fig:diagram} shows an example: the question that asks how many sides a brick has can be transformed into more explicit reasoning over a given fact, \textsl{\uline{A brick is a cube.}} (Assuming that the model readily knows that a cube has six faces.)
\autoref{tab:qualitative} shows more such examples across different datasets, with how the prediction is influenced by the additional knowledge.
In this sense, when faced with questions that requires commonsense, the model may be implicitly performing two jobs together: (1) to come up with \textit{ground knowledge}, i.e. knowledge statements that are helpful in reasoning about the question, and (2) to perform reasoning based on such knowledge.
Our hypothesis is that breaking this down into two explicit steps, namely knowledge generation and knowledge-prompted inference, would unleash the model capacity so it can focus on an explicit and knowledge-grounded reasoning procedure.
While some existing work also leverage certain types of model-generated text to improve performance on commonsense reasoning \cite{shwartz-etal-2020-unsupervised, paranjape-etal-2021-prompting, bosselut2021dynamic}, we focus on generating and prompting knowledge that can explicitly support the reasoning process in a general way.

% A few existing work have shown that PLMs can leverage certain types of text generated by themselves to improve their CSR inference performance \cite{shwartz-etal-2020-unsupervised, paranjape-etal-2021-prompting, bosselut2021dynamic}.
% However, these methods are inefficient, domain-restricted, and/or require heavy domain expertise and engineering efforts to transfer.
% We would like to have a knowledge generation process that is flexible enough to generate diverse types of knowledge, so that the generated knowledge stays relevant to the domain.
% While these methods are often built upon thinking of what kinds of knowledge \textit{can} be generated, \yejin{I am not sure this statement is a particularly accurate summary of the prior work... did prior work explore the scope of knowledge that "can be" generated?} we take a different approach by reflecting on what kinds of knowledge are \textit{needed}. \yejin{prior work compared also study what knowledge "need to be" generated in some sense. Hanna/Bhargavi's paper for example demonstrate that contrastive knowledge need to be generated? can we find a different angle that is more accurate and crisp?}
% These methods often make \textit{a priori} assumptions on the type of knowledge to generate, and use them to control the generation process, leading to knowledge that may be only loosely relevant to answering the question.
% To address this, we take an approach by first reflecting on what are the commonalities of knowledge that are the most relevant to CSR, and then proposing a generic framework that systematically generates and utilizes such knowledge across various CSR domains.
% We hypothesize that many CSR problems can be reduced to more basic types of reasoning over \textit{ground knowledge} -- sentences that can serve as the premises for some reasoning process.
% For instance, in \autoref{fig:diagram} the commonsense question, which asks how many sides a brick has, can become a deductive reasoning problem when given the premise \textsl{\uline{A brick is a cube}}. (Assuming that the model knows that a cube has six faces.)
% The examples in \autoref{tab:qualitative} show how CSR problems from various datasets can, when provided with the appropriate knowledge, be reduced to different reasoning types such as deduction, induction, analogy, and paraphrasing.
% For example, in \S\ref{sec:numersense} we show that numerical CSR problems can, when provided with the appropriate premises, be reduced to straightforward reasoning types such as deduction, induction, paraphrasing, etc.
% In this sense, when answering a CSR question, the model may be implicitly performing two jobs together: (1) to come up with the knowledge that are helpful to answering the question, and (2) to reason with such knowledge.
% Breaking this down into two explicit steps, namely knowledge generation and knowledge-augmented inference, would unleash the model capacity so it can focus on a reduced form of reasoning.

In this work, we present the Generated Knowledge Prompting framework that follows this approach.
We take the pretrained language models off-the-shelf, elicit question-related ground knowledge  from these models, and augment the question with such knowledge before sending it to the model for inference.
This process is unsupervised and resource-efficient, since we do not need a training set to finetune the knowledge generation or inference model, or an in-domain knowledge base to retrieve knowledge from.
It is also more generic and engineering-efficient compared to previous methods, making it easily adaptable to various tasks.
% Generated Knowledge Prompting would be particularly beneficial for nascent, low-resource commonsense reasoning tasks where there is no or little training data to properly finetune the model with, and no appropriate knowledge base from which to retrieve relevant knowledge.
% Such scenario is conceivable either with a new diagnostic CSR benchmark, or a production QA system where incoming user queries may not fit in the domain of any existing CSR dataset.

We apply our method on recently released commonsense reasoning datasets -- NumerSense, CommonsenseQA, CommonsenseQA 2.0, and QASC -- and demonstrate that we can push the limits of existing models. % with only lightweight engineering efforts, and without any extra data collection or model optimization steps.
Our method improves the state-of-the-art of NumerSense by about 9\%, and that of CommonsenseQA 2.0 by about 2\%.
It also shows superior performance over the state-of-the-art generative knowledge approach, self-talk \cite{shwartz-etal-2020-unsupervised}, and is comparable to retrieval-based methods.
Experimental results show that our method is effective under a variety of settings: with different sizes of knowledge generation models and inference models, and with both zero-shot and finetuned inference models.
In particular, it is effective even when knowledge generation and inference are done with the same base language model.

% So does Generated Knowledge Prompting work so well for the reason we think it does?
% That is to say, are the generated knowledge truly providing grounds for reasoning?
% \name{} can be perceived as a type of symbolic knowledge transfer if we use the knowledge generated by a larger model to improve a smaller inference model.
% However, it is not very intuitive as to why performance also improves when knowledge generation and inference are done with the same model.
% If knowledge are encoded implicitly in the neural components of the PLM, how come generating them symbolically be helpful for inference?
% To understand this, we conduct a quantitative study of the behavior of the inference model (\S\ref{sec:analysis}).
Through a quantitative study of the behavior of the inference model (\S\ref{sec:analysis}), we find that two factors contribute to the method's success: the high quality of the generated knowledge, and ensembling over the predictions of many knowledge statements.
Furthermore, qualitative analysis (\S\ref{sec:qualitative}) also shows that the generated knowledge can reduce commonsense question answering to certain explicit reasoning procedures using the generated knowledge. % serves to reduce the reasoning process in ways that we expected, and even enables new reasoning types that we did not anticipate.
% Our intuition is that by explicating ground knowledge through symbolic generation, the model can incorporate the knowledge with full certainty and thus perform more deterministic knowledge-grounded reasoning.
% We hope that the insights we share will inspire further efforts on improving the robustness and explainability of PLM-based inference.
Our work shows a novel yet important role of symbolic representation of knowledge in the neural reasoning process, and we hope that the insights we share will inspire further efforts on neuro-symbolic knowledge integration.

==> atrash/numersense.tex <==
\section{A Case Study with Numerical Commonsense}
\label{sec:numersense}

\alisainline{There should be a table that shows examples of generated knowledge for each dataset. This has the benefit of giving an example from each dataset to illustrate the task, as well as showing what model's generative capabilities are. I think it would be a good Page 2 table, even if it's referenced much later on in the experiments.}

We first conduct a case study on the NumerSense dataset \cite{lin-etal-2020-birds} to show how ground knowledge prompts models to perform better on commonsense inference.%, and how we can generate such relevant knowledge.

NumerSense challenges models on the task of numerical commonsense reasoning.
It presents generic statements about common concepts while masking a number token in each sentence, which the model needs to recover.
The masked numbers are always integers between zero and ten (inclusive), so NumerSense can be formulated as a multiple-choice task.

We analyze a strong baseline model on NumerSense based on T5-11B.
Although it achieves a very high performance on the leaderboard, this model still makes numerous mistakes on very simple questions.
Consider the following question from the dev set:
\begin{center}\textbf{Most motorcycles have [M] tires.}\end{center}
T5-11B predicts \textcolor{wrong}{four} as an answer with a confidence of \textcolor{wrong}{0.33}, whereas the correct answer \textcolor{right}{two} only gets a confidence of \textcolor{right}{0.32}.
However, if we prepend the following knowledge sentences to this question:
\begin{center}\textsl{A motorcycle has two wheels. Each wheel has a tire.}\end{center}
The inference model then assigns a high confidence (\textcolor{right}{0.86}) to the correct answer \textcolor{right}{two} and thus make the right prediction.
Note that the question and the context form a deductive reasoning process, where the question is the conclusion and the two additional sentences serve as the premises.
The addition of knowledge essentially reduces this commonsense problem to a deductive reasoning problem.
Furthermore, we observe that using only one of these two premises as the context is also able to rectify the prediction (\autoref{tab:numersense_qual}), demonstrating that the inference model can incorporate partially-complete premise set into its reasoning process.

Based on the question of interest, there can be different kinds of ground knowledge, and they can transform the type of reasoning required in different ways.
\autoref{tab:numersense_qual} shows more examples where manually-written knowledge rectifies the prediction.
Ground knowledge can be numerical (e.g. \textsl{\uline{A cube has eight vertices.}}), attributive (e.g. \textsl{\uline{Triangles are polygons with the least number of sides.}}), and taxonomical (e.g. \textsl{\uline{Scallop is a kind of clam.}}).
The reduced reasoning types may be straightforward paraphrasing, logical reasoning such as deduction and induction, numerical reasoning such as counting and arithmetics, etc.

With this observation, we pose the next research question: can we use models to generate ground knowledge that are still able to rectify the model predictions?
In the next section, we introduce a framework for knowledge generation and prompting which answers this question with a resounding yes.

==> atrash/qasc_hist.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{floats/qasc_hist.png}
\caption{
    Distribution of some metrics of inference probabilities under different input augmentation methods.
    This is an alternative view of \autoref{fig:qasc_scatter}.
    We compute the mean and standard deviation of inference probabilities under all augmentation texts for each example, and plot a histogram of these metrics across all examples (the first and second rows, respectively).
    We also plot a histogram of the inference probability under the selected augmentation text for each example (the third row).
    The (\textcolor{right}{green} and \textcolor{wrong}{red}) solid vertical lines stand for the mean of these metrics, whereas the dashed vertical lines are the mean of such metrics on the no-augmentation baseline.
}
\label{fig:qasc_hist}
\end{figure*}

==> atrash/qasc_scatter.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{floats/qasc_scatter.png}
\caption{
    Impact of input augmentation methods on inference probabilities.
    Each plot is a scatter plot that shows the change in inference probability with some input augmentation method.
    The horizontal axis is the inference probability without input augmentation, and the vertical axis is the inference probability with an augmentation text.
    We plot the impact of each augmentation text on every example in the QASC dev set.
    The \textcolor{yellow}{yellow} dots show all $M$ augmentations for each example, and the \textcolor{right}{green} or \textcolor{wrong}{red} dots show the augmentation selected by the max-ensembling algorithm to make the final prediction.
    The first row of plots show the impact on \textcolor{right}{correct answers}, whereas the second row show the impact on \textcolor{wrong}{distractors}.
    We present results for the following input augmentation methods: Language Augmentation, Context Augmentation, and Knowledge Augmentation with model-generated knowledge or gold knowledge.
    We use $M=20$ for methods with model-generated augmentations, and $M=1$ or $2$ for methods using gold knowledge as augmentations.
    The legend shows the mean inference probability.
    The right-most column of plots is special: it shows the impact of finetuning instead of input augmentation. 
    The vertical axis is the inference probability from a finetuned T5-11b model with no input augmentation.
}
\label{fig:qasc_scatter}
\end{figure*}

==> atrash/qasc_summary.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{floats/qasc_summary.png}
\caption{
    Inference model behavior under different types of prompts.
    Measured on the QASC dev set with T5-11b as the inference model.
    Generated Knowledge Prompting is denoted by Knowledge ($K$), whereas other types of prompts are described in \S\ref{sec:analysis}.
    For each type of prompt, we show the mean of induced average (dashed lines), mean of induced deviation (filled areas), and selected score (solid lines) for \textcolor{right}{correct answers} and \textcolor{wrong}{distractors}.
    We also plot the \textcolor{blue}{prediction accuracy} given by the inference model.
}
\label{fig:qasc_summary}
\end{figure*}

==> atrash/qual_numersense.tex <==
\begin{table*}[t]
\footnotesize
\centering
\begin{tabular}{p{9.5cm}|ccc}
\toprule
\textbf{Question} / \textsl{Knowledge} & \textbf{Prediction} & \textbf{Confidence} & \textbf{Reasoning} \\
\midrule
\textbf{most motorcycles have [M] tires.} & \textcolor{wrong}{four} & \textcolor{wrong}{0.33} | \textcolor{right}{0.32} & CSR \\
\qquad \textsl{Each wheel has a tire.} & \textcolor{right}{two} & \textcolor{right}{0.53} & Deduction \\
\qquad \textsl{A motorcycle has two wheels.} & \textcolor{right}{two} & \textcolor{right}{0.70} & Deduction \\
\qquad \textsl{A motorcycle has two wheels. Each wheel has a tire.} & \textcolor{right}{two} & \textcolor{right}{0.86} & Deduction \\
\midrule
\textbf{any closed two-dimensional shape must have at least [M] sides.} & \textcolor{wrong}{two} & \textcolor{wrong}{0.27} | \textcolor{right}{0.18} & CSR \\
\qquad \textsl{Triangles are polygons with the least number of sides.} & \textcolor{right}{three} & \textcolor{right}{0.85} & Deduction \\
\midrule
\textbf{clams have evolved to have [M] shells.} & \textcolor{wrong}{no} & \textcolor{wrong}{0.37} | \textcolor{right}{0.18} & CSR \\
\qquad \textsl{Scallop is a kind of clam. A scallop has two shells.} & \textcolor{right}{two} & \textcolor{right}{0.53} & Induction \\
\midrule
\textbf{a normal cube has [M] corners.} & \textcolor{wrong}{six} & \textcolor{wrong}{0.47} | \textcolor{right}{0.15} & CSR \\
\qquad \textsl{A cube has eight vertices.} & \textcolor{right}{eight} & \textcolor{right}{0.40} & Paraphrasing \\
\midrule
\textbf{a game of chess may have [M] outcomes.} & \textcolor{wrong}{two} & \textcolor{wrong}{0.48} | \textcolor{right}{0.08} & CSR \\
\qquad \textsl{In a game of chess, we can win, or lose, or draw with the opponent.} & \textcolor{right}{three} & \textcolor{right}{0.51} & Counting \\
\midrule
\textbf{a proton is made of [M] independent quarks.} & \textcolor{wrong}{six} & \textcolor{wrong}{0.34} | \textcolor{right}{0.30} & CSR \\
\qquad \textsl{A proton is made of two up quarks and one down quark.} & \textcolor{right}{three} & \textcolor{right}{0.92} & Arithmetic \\
\bottomrule
\end{tabular}
\caption{
    Examples from NumerSense dev set where additional knowledge rectifies the prediction.
    The first row of each section is the original question and the inference results associated with it, followed by manually-written knowledge text that are prepended before the question during inference.
    We show \textcolor{right}{correct predictions in green}, \textcolor{wrong}{incorrect predictions in red}, and their corresponding confidence values produced by the model.
}
\label{tab:numersense_qual}
\end{table*}

==> atrash/results.tex <==
\begin{table*}[t]
% \footnotesize
\centering
\begin{tabular}{c|ccc|c|cc|cc}
\toprule
\textbf{Task} & \multicolumn{3}{c}{\textbf{NumerSense}} & \textbf{CSQA} & \multicolumn{2}{c}{\textbf{CSQA2}} & \multicolumn{2}{c}{\textbf{QASC}} \\
\midrule
Inference & \multicolumn{3}{c}{T5-11b} & T5-11b & \multicolumn{2}{c}{Unicorn-11b-ft} & \multicolumn{2}{c}{T5-11b} \\
& \textit{dev} & \textit{test-core} & \textit{test-all} & \textit{dev} & \textit{dev} & \textit{test} & \textit{dev} & \textit{test} \\
\midrule
\textbf{Baseline} & 67.5 & 70.23 & 64.08 & 39.89 & 69.9 & 70.2 & 48.16 & 44.89 \\
\rowcolor{ours}
\textbf{ours} & \textbf{78.0} & \textbf{79.24} & \textbf{72.47} & \textbf{47.26} & \textbf{72.37} & \textbf{73.03} & \textbf{58.32} & \textbf{55.00} \\
\bottomrule
\end{tabular}
\caption{
    An overview of empirical results across all tasks.
    \textbf{ours}: Generated Knowledge Prompting, which is highlighted in green (same below).
    For our method, knowledge are generated by GPT3 for all datasets.
    All tasks use the off-the-shelf T5-11b model for inference, except for CSQA2 where we use a finetuned version of Unicorn-11b.
}
\label{tab:results}
\end{table*}

==> atrash/results_csqa.tex <==
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{cc|c}
\toprule
\multicolumn{3}{c}{\textbf{CSQA}} \\
\midrule
\textbf{Inference} & \textbf{Knowledge} & \textbf{dev} \\
\midrule
T5-11b & -- & 39.89 \\
T5-11b & self-talk (GPT3) & 45.37 \\
\rowcolor{ours}
T5-11b & GPT3 & \textbf{47.26} \\
\midrule
UQA-11b & -- & 76.99 \\
UQA-11b & self-talk (GPT3) & 77.97 \\
\rowcolor{ours}
UQA-11b & GPT3 & \textbf{78.71} \\
% \midrule
% T5-11b-ft & -- & 83.54 & \textcolor{red}{TODO} \\
% T5-11b-ft & GPT3 & \textbf{83.78} & \textcolor{red}{TODO} \\
% \midrule
% UQA-11b-ft & -- & 85.18 & \textcolor{red}{TODO} \\
% UQA-11b-ft & GPT3 & \textbf{85.34} & \textcolor{red}{TODO} \\
\midrule
\multicolumn{2}{c}{Prev. SOTA$^\ddagger$} & 81.8 \\
\bottomrule
\end{tabular}
\caption{
    Detailed empirical results on CSQA.
    \textbf{UQA}: the UnifiedQA model.
    $\ddagger$: ALBERT + SFR (prev. SOTA with no reference to ConceptNet).
}
\label{tab:results_csqa}
\end{table}

==> atrash/results_csqa2.tex <==
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{cc|cc}
\toprule
\multicolumn{4}{c}{\textbf{CSQA2}} \\
\midrule
\textbf{Inference} & \textbf{Knowledge} & \textbf{dev} & \textbf{test} \\
\midrule
Unicorn-11b-ft & --$^\ddagger$ & 69.9$^\ddagger$ & 70.2$^\ddagger$ \\
\rowcolor{ours}
Unicorn-11b-ft & GPT3 & \textbf{72.37} & \textbf{73.03} \\
\midrule
Unicorn-11b-ft & Google snippets$^\dagger$ & 74.0$^\dagger$ & 73.3$^\dagger$ \\
\bottomrule
\end{tabular}
\caption{
    Detailed empirical results on CSQA2.
    $\ddagger$: Finetuned Unicorn-11b baseline by \citet{talmor2021commonsenseqa} (prev. SOTA without Google retrieval).
    $\dagger$: Knowledge prompting with Google-retrieved snippets \cite{talmor2021commonsenseqa}.
}
\label{tab:results_csqa2}
\end{table}

==> atrash/results_numersense.tex <==
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{cc|ccc}
\toprule
\multicolumn{5}{c}{\textbf{NumerSense}} \\
\midrule
\textbf{Inference} & \textbf{Knowledge} & \textbf{dev} & \textbf{test-core} & \textbf{test-all} \\
\midrule
T5-11b & --$^{*}$ & 67.5 & 70.23$^{*}$ & 64.08$^{*}$ \\
T5-11b & IR$^{\dagger}$ & -- & 70.41$^{\dagger}$ & 65.10$^{\dagger}$ \\
\multicolumn{2}{c}{Prev. SOTA$^{\ddagger}$} & -- & 72.61$^{\ddagger}$ & 66.18$^{\ddagger}$ \\
\rowcolor{ours}
T5-11b & GPT3 & \textbf{78.0} & \textbf{79.24} & \textbf{72.47} \\
\midrule
GPT3 & -- & 72.0 & 74.91 & 66.34 \\
\rowcolor{ours}
GPT3 & GPT3 & \textbf{81.0} & \textbf{80.74} & \textbf{73.46} \\
\bottomrule
\end{tabular}
\caption{
    Detailed empirical results on NumerSense with different knowledge sources and inference models.
    *: T5-11b baseline \cite{stanford}.
    $\dagger$: Information retrieval method \cite{uscink}.
    $\ddagger$: Submission by ISI Waltham.
    Leaderboard retrieved on 09/09/2021.
}
\label{tab:results_numersense}
\end{table}

==> atrash/results_qasc.tex <==
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{cc|cc}
\toprule
\multicolumn{4}{c}{\textbf{QASC}} \\
\midrule
\textbf{Inference} & \textbf{Knowledge} & \textbf{dev} & \textbf{test} \\
\midrule
T5-11b & -- & 48.16 & 44.89 \\
\rowcolor{ours}
T5-11b & GPT3 & \textbf{58.32} & \textbf{55.00} \\
\midrule
UQA-11b & -- & 67.93 & 67.07 \\
\rowcolor{ours}
UQA-11b & GPT3 & \textbf{74.41} & \textbf{75.33} \\
\midrule
T5-11b-ft & -- & 76.03 & 73.91 \\
\rowcolor{ours}
T5-11b-ft & GPT3 & \textbf{78.62} & \textbf{77.17} \\
\midrule
UQA-11b-ft & -- & 81.75 & 76.74 \\
\rowcolor{ours}
UQA-11b-ft & GPT3 & \textbf{84.02} & \textbf{80.33} \\
\midrule
\multicolumn{2}{c}{Prev. SOTA$^\ddagger$} & -- & 89.57 \\
\bottomrule
\end{tabular}
\caption{
    Detailed empirical results on QASC.
    \textbf{UQA}: the UnifiedQA model.
    $\ddagger$: UQA-11b-ft + IR (prev. SOTA).
}
\label{tab:results_qasc}
\end{table}

==> atrash/theory.tex <==
\section{A Theoretical Perspective}

In this section, we make an attempt to explain why knowledge augmentation works so well.
We will present some theories, and show quantitative analysis with QASC in support of these theories.

The method we will look at is Input Augmentation (IA), which is a generalization of UKA and contains two weaker alternatives to it: Context Augmentation (CA) and Language Augmentation (LA).
All these method involves extending the input with a piece of text.
The difference is that the augmentation text in CA and LA may not be as relevant as UKA.
In particular, CA augments the input with a piece of text sampled from the context of the input, and LA does so by freely sampling some text from the language model without conditioning on the input.
We introduce these alternatives as they provide simpler mathematical interface than UKA.

\subsection{Preliminaries}

Suppose we have a dataset $D = \{(x, y)\}$, where $x \in X$ is the input text and $y \in Y$ is the desired output text, and an inference language model $p(y|x)$.
The model decides the best output with $\hat{y} = \argmax_{y \in Y}{p(y|x)}$.

During IA, we prepend a piece of text $z \in Z$ before the input $x$, so that the inference process can be written as $p(y|z,x)$.
In practice, a set of augmentation texts $Z_e$ are sampled, and prediction results produced by augmenting each $z \in Z_e$ are ensembled to derive the final prediction:
\begin{align*}
z^* &= \argmax_{z \in Z_e}{\max_{y \in Y}{p(y|z,x)}} \\
\hat{y} &= \argmax_{y \in Y}{p(y|z^*,x)}
\end{align*}

Conceptually, $X = Y = Z = L$, where $L$ is the space of natural language texts.
We will use this setting for our theoretical analysis.
However, for empirical analysis with the QASC dataset, we restrict $Y = Y_q$, the list of choices for each question in QASC, and $Z = Z_e$ because it is intractable to marginalize over the entire text space.
We normalize the inference probabilities over the reduced output space:
\begin{align*}
\tilde{p}(y|x) &= \frac{p(y|x)}{\sum_{y' \in Y_q}{p(y'|x)}} \\
\tilde{p}(y|z,x) &= \frac{p(y|z,x)}{\sum_{y' \in Y_q}{p(y'|z,x)}}
\end{align*}

\subsection{An assumption with language models}

For simplicity, assume that we work with an autoregressive LM.
We define the joint probability and conditional probability of pairs of texts w.r.t. the LM as
\begin{align*}
p(x,y) &\equiv p([x || y]) \\
p(y|x) &\equiv \frac{p(x,y)}{p(x)} \equiv \frac{p([x || y])}{p(x)}
\end{align*}

We make the assumption that the LM satisfies the following equation:
\begin{align*}
p(a) &= \sum_{b \in L}{p(b) p(a|b)} \equiv \sum_{b \in L}{p(b,a)} \equiv \sum_{b \in L}{p([b || a])}
\end{align*}
This is the foundation of our theoretical analysis below.
I guess this is not strictly true for LMs, and we need to look into how close it is to real LMs, but I suppose this provides a reasonable approximation that greatly simplifies our further discussion.

\subsection{Language and Context Augmentation}

For a given example $(x, y) \in D$, in Language Augmentation we arbitrarily sample the augmentation text from the LM: $z \sim p(\cdot)$; whereas in Context Augmentation we sample it from the context (a.k.a. continuation) of the input: $z \sim p(\cdot|x)$.

\subsubsection{Conservation of expectation of inference probabilities}
\label{sec:expectation}

For Context Augmentation, the expectation of probability assigned by the inference model to the desired output is equal to that without IA.
Formally,
\begin{align*}
p(y|x) &= \sum_{z \in L}{p(z|x) p(y|z,x)} = \mathbb{E}_{z \sim p(\cdot|x)}{\big[ p(y|z,x) \big]}
\end{align*}
This also applies to the desired output $y$ any distractor $y' \in L$.
Therefore, if only one augmentation text is generated, Context Augmentation does not improve the model's confidence on the correct answer on average.

\textcolor{red}{TODO: Similar result for LAug?}

% Note, however, that if we compute the expectation of model loss (i.e. negative log likelihood, NLL), Context Augmentation is guaranteed to increase the loss value:
% \begin{align*}
% L(y;x) &= -\log{p(y|x)} \\
% &= -\log{\sum_{z \in L}{p(z|x) p(y|z,x)}} \\
% &\le \sum_{z \in L}{p(z|x) \big[ -\log{p(y|z,x)} \big]} & \text{(Jensen's inequality)} \\
% &= \mathbb{E}_{z \sim p(\cdot|x)}{\big[ L(y;z,x) \big]}
% \end{align*}
% which does not give us a stable baseline to investigate the effect of input augmentation, so we do not use this metric.

\subsubsection{(Differential) increase of variance of inference probabilities}
\label{sec:variance}

Although LA and CA are shown not to make the inference model more confident on the desired outputs, they can create an intrinsic variance within such confidence by introducing multiple augmentation texts.
The naive inference process assigns a single confidence score to each output for a given input: $p(y|x)$.
In comparison, IA produces a list of confidence scores:
\begin{align*}
\big[ p(y|z_1,x), \hdots, p(y|z_m,x), \hdots, p(y|z_M,x) \big]
\end{align*}
where $Z_e = \{z_1, \hdots, z_M\}$.

Through the quantitative analysis, we will empirically show that the variance of these confidence scores tends to be larger for desired outputs than distractors:
\begin{align*}
\mathbb{E}_{(x,y),Z_e}{\Big[\text{Std}\big[\{p(y|z_i,x)\}\big]\Big]} \\
> \mathbb{E}_{(x,y),y',Z_e}{\Big[\text{Std}\big[\{p(y'|z_i,x)\}\big]\Big]}
\end{align*}
One hypothesis is that, for desired outputs, the evidences/explanations/justifications in support of these outputs can make reasoning more convincing.\footnote{Though this also means that those evidence in contradiction with these outputs are more convincing as well.}

As a result, desired outputs tend to contain more \textit{extreme} confidence values under IA.
This implies that the max-ensembling algorithm, which uses the augmentation that most strongly supports any output, tends to pick up augmentations that result in high confidence values on the desired output.

\subsubsection{Reduction of entropy in output space}
\label{sec:entropy}

Now we take a look at the change of entropy of output space due to IA.
The entropy of output space without IA is $\mathcal{H}(Y|x)$, and the entropy with IA is $\mathcal{H}(Y|Z,x)$.
The change is equal to
\begin{align*}
\mathcal{H}(Y|Z,x) - \mathcal{H}(Y|x) &= -\mathcal{I}(Y;Z|x)
\end{align*}
which is the mutual information of output variable $Y$ and augmentation variable $Z$ for a given input $x$.

For LA, $Z \sim p(\cdot)$ is sampled freely from the LM, so it has zero mutual information with $Y$.
Therefore, LA does not change the entropy of output space.

For CA, $Z \sim p(\cdot|x)$ is sampled conditioning on the input $x$, so $Z$ is correlated to $Y$, and thus the mutual information $\mathcal{I}(Y;Z|x)$ is positive.
Therefore, CA reduces the entropy of output space.

\subsection{Quantitative analysis on QASC}

\input{floats/results_qasc_hierarchy}
\input{floats/qasc_scatter}
\input{floats/qasc_hist}

In QASC, each example comes with a fact sentence that can directly answer the question; this sentence is in turn formed by the composition of two separate \textit{fact} sentences, which are also provided in the dataset.
In some sense, these sentences can be regarded as the best possible augmentations, so that we can see the upperbound of capability of IA.

We run inference on the QASC dev set with the off-the-shelf T5-11b and UnifiedQA-T5-11b models, using the following input augmentation methods:
\begin{enumerate}
\item Language Augmentation. For each example, we use GPT2-large to sample $M=20$ random sentences, without looking at the content of question or choices.
\item Context Augmentation. For each example, we use GPT2-large to sample $M=20$ continuations to the question. The generated sentences can be seen as a representative set of context sentences wrt the question sentence.
\item Knowledge Augmentation. For each example, we use GPT3 to generate up to $M=20$ knowledge sentences based on the keywords in the question, using a few-shot, in-context learning prompt.
\item Knowledge Augmentation with gold, separate knowledge. In this case we use the two \textit{fact} sentences associated with the question as augmentation texts, and thus $M=2$.
\item Knowledge Augmentation with gold, combined knowledge. In this case we use the composition \textit{fact} sentence associated with the question as augmentation texts, and thus $M=1$.
\end{enumerate}

\autoref{fig:qasc_scatter} shows the impact of these input augmentation methods on inference probabilities for correct answers and distractors.
See the caption for explanation of these plots.
Ideally, we would like to see points to fall into the upper-left triangle for correct answers, and into the lower-right triangle for distractors, which would manifest that we are pushing the model to be more confident on correct answers.
The plots for finetuned T5 inference model clearly shows such a trend, where the dots in the answer plot (first row) are densely aggregated around the $y=1$ line, and the dots in the distractor plot (second row) around the $y=0$ line.
KA with gold facts, either separate or combined, also shows a similar trend, and the average of inference probabilities moves accordingly (up for correct answers, down for distractors).
If we focus on the \textcolor{right}{green} and \textcolor{wrong}{red} dots, which shows the impact of the augmentation text selected by the max-ensembling algorithm, the trend is even more apparent, and the magnitude of change in average model confidence is also magnified.
This proves the effectiveness of IA when working with best possible augmentation text -- the upperbound is high.

For KA with model-generated augmentation texts, we see the same trend with milder magnitude -- the average inference probabilities still change considerably while not as much as KA with oracle augmentation texts.
LA and CA, on the other hand, show no significant change on average inference probabilities when considering all augmentation texts, which is consistent with our theory in \S\ref{sec:expectation}.
Interestingly, if we only consider the selected augmentation texts, there is still an improvement to the inference probabilities over the baseline.

We observe that IA methods tend to create more extreme inference probabilities.
The dots tend to be pushed towards the upper ($y=1$) and lower ($y=0$) areas of the plots, whereas the area in the middle is relatively sparse.
The existence of such phenomenon indirectly manifests the reduction of entropy in output space in \S\ref{sec:entropy}.
This phenomenon is stronger for correct answer than for distractors, which is mentioned in \S\ref{sec:variance}.
Also, this phenomenon is stronger for selected augmentation texts.

Perhaps the differential increase of variance of inference probabilities is more evident in \autoref{fig:qasc_hist}.
The second row plots the distribution of standard deviation of inference probabilities induced by augmentation.
As we can see, under all input augmentation methods, the induced variance tend to be larger for correct answers than distractors.

\subsection{Summary}

\input{floats/theory_summary}

\autoref{tab:theory_summary} summarizes our findings, namely:
\begin{enumerate}
\item Language and Context Augmentation does not change the expectation of inference probabilities. However, empirical results show that Knowledge Augmentation tends to increase the model's confidence on desired outputs (i.e. correct answers), and decrease the model's confidence on undesired outputs (i.e. distractors).
\item Input Augmentation methods create an intrinsic variance on the inference probabilities. Empirical results show that this variance tends to be larger for desired outputs than undesired outputs. This, together with our max-ensembling algorithm, makes the desired outputs more favorable for the inference model.
\item Input Augmentation methods reduce the entropy of the output space. Though this does not guarantee that the desired outputs get more favorited than undesired outputs.
\end{enumerate}

==> atrash/theory_summary.tex <==
\begin{table}[t]
\centering
\begin{tabular}{c|cc|cc|c}
\toprule
\textbf{Method} & \multicolumn{2}{c}{\textbf{$\mu$}} & \multicolumn{2}{c}{\textbf{$\sigma$}} & \textbf{$\mathcal{H}$} \\
& \textbf{\cmark} & \textbf{\xmark} & \textbf{\cmark} & \textbf{\xmark} & \\
\midrule
Language Augmentation & \multicolumn{2}{c}{--} & \textcolor{magenta}{$\uparrow$}$\uparrow$ & \textcolor{magenta}{$\uparrow$} & \textcolor{magenta}{--} \\
Context Augmentation & \multicolumn{2}{c}{\textcolor{magenta}{--}} & \textcolor{magenta}{$\uparrow$}$\uparrow$ & \textcolor{magenta}{$\uparrow$} & \textcolor{magenta}{$\downarrow$} \\
Knowlegde Augmentation & $\uparrow$ & $\downarrow$ & \textcolor{magenta}{$\uparrow$}$\uparrow$ & \textcolor{magenta}{$\uparrow$} & \textcolor{magenta}{$\downarrow$} \\
\bottomrule
\end{tabular}
\caption{
    Summary of UKA theory and quantitative analysis.
    Black means observed in empirical results but have no theoretical proof; \textcolor{magenta}{magenta} means both observed in empirical results and we have a theoretical proof.
}
\label{tab:theory_summary}
\end{table}

==> floats/qualitative_short.tex <==
\begin{table*}[t]
\footnotesize
\centering
\begin{tabular}{cp{7cm}ccc}
\toprule
\textbf{Dataset} & \textbf{Question} / \textsl{Knowledge} & \textbf{Prediction} & \textbf{Reasoning} \\
% \midrule
% \multirow{2}{*}{NumerSense} & \textbf{clams have evolved to have [M] shells.} & \textcolor{wrong}{no} & \textcolor{wrong}{0.37} | \textcolor{right}{0.18} & \textcolor{gray}{Commonsense} \\
% & \qquad \textsl{Clams have a bivalve shell.} & \textcolor{right}{two} & \textcolor{right}{0.89} & Paraphrasing \\
\midrule
\multirow{2}{*}{NumerSense} & \textbf{an easel can have [M] or four legs.} & \textcolor{wrong}{two} & \textcolor{gray}{Commonsense} \\
& \qquad \textsl{A tripod is a kind of easel.} & \textcolor{right}{three} & Induction \\
% \midrule
% \multirow{2}{*}{NumerSense} & \textbf{bricks are [M] sided.} & \textcolor{wrong}{four} & \textcolor{wrong}{0.27} | \textcolor{right}{0.13} & \textcolor{gray}{Commonsense} \\
% & \qquad \textsl{A brick is a cube.} & \textcolor{right}{six} & \textcolor{right}{0.71} & Deduction \\
% \midrule
% \multirow{2}{*}{NumerSense} & \textbf{the word children means [M] or more kids.} & \textcolor{wrong}{one} & \textcolor{wrong}{0.37} | \textcolor{right}{0.35} & \textcolor{gray}{Commonsense} \\
% & \qquad \textsl{The word child means one kid.} & \textcolor{right}{two} & \textcolor{right}{0.91} & Analogy \\
\midrule
\multirow{2}{*}{CSQA} & \textbf{Where does a heifer's master live?} & \textcolor{wrong}{slaughter house} & \textcolor{gray}{Commonsense} \\
& \qquad \textsl{The master of a heifer is a farmer.} & \textcolor{right}{farm house} & Deduction \\
% \midrule
% \multirow{2}{*}{CSQA} & \textbf{Aside from water and nourishment what does your dog need?} & \textcolor{wrong}{walked} & \textcolor{wrong}{0.55} | \textcolor{right}{0.04} & \textcolor{gray}{Commonsense} \\
% & \qquad \textsl{Dogs need attention and affection.} & \textcolor{right}{lots of attention} & \textcolor{right}{0.91} & Elimination \\
% \midrule
% \multirow{2}{*}{CSQA} & \textbf{What is the result of applying for job?} & \textcolor{wrong}{praise} & \textcolor{wrong}{0.98} | \textcolor{right}{0.02} & \textcolor{gray}{Commonsense} \\
% & \qquad \textsl{The result of applying for a job is that you get a job.} & \textcolor{right}{being employed} & \textcolor{right}{0.99} & Paraphrasing \\
\midrule
\multirow{2}{*}{CSQA} & \textbf{I did not need a servant. I was not a what?} & \textcolor{wrong}{in charge} & \textcolor{gray}{Commonsense} \\
& \qquad \textit{People who have servants are rich.} & \textcolor{right}{rich person} & Abduction \\
% \midrule
% \multirow{2}{*}{CSQA2} & \textbf{Part of golf is trying to get a higher point total than others.} & \textcolor{wrong}{yes} & \textcolor{wrong}{1.00} | \textcolor{right}{0.00} & \textcolor{gray}{Commonsense} \\
% & \qquad \textit{The player with the lowest score wins.} & \textcolor{right}{no} & \textcolor{right}{1.00} & Negation \\
% \midrule
% \multirow{2}{*}{CSQA2} & \textbf{If a piece of lead and a feather are falling thought vacuum, none will reach the bottom earlier.} & \textcolor{wrong}{no} & \textcolor{wrong}{0.59} | \textcolor{right}{0.41} & \textcolor{gray}{Commonsense} \\
% & \qquad \textit{All objects fall at the same rate in a vacuum.} & \textcolor{right}{yes} & \textcolor{right}{1.00} & Deduction \\
% \midrule
% \multirow{2}{*}{CSQA2} & \textbf{A minute will pass only if sixty seconds have passed.} & \textcolor{wrong}{no} & \textcolor{wrong}{1.00} | \textcolor{right}{0.00} & \textcolor{gray}{Commonsense} \\
% & \qquad \textit{A minute is a unit of time equal to 60 seconds.} & \textcolor{right}{yes} & \textcolor{right}{1.00} & Paraphrasing \\
% \midrule
% \multirow{2}{*}{CSQA2} & \textbf{Eighth plus eight is smaller than fifteen.} & \textcolor{wrong}{yes} & \textcolor{wrong}{0.97} | \textcolor{right}{0.03} & \textcolor{gray}{Commonsense} \\
% & \qquad \textit{Eighth plus eight is sixteen, which is larger than fifteen.} & \textcolor{right}{no} & \textcolor{right}{1.00} & Numerical \\
\midrule
\multirow{2}{*}{QASC} & \textbf{[M] is used for transportation.} & \textcolor{wrong}{plastic} & \textcolor{gray}{Commonsense} \\
& \qquad \textit{Bicycles are used for transportation.} & \textcolor{right}{boats} & Analogy \\
% \midrule
% \multirow{2}{*}{QASC} & \textbf{Hydrostatic skeletons are a feature of some [M].} & \textcolor{wrong}{eukaryotic cells} & \textcolor{wrong}{0.46} | \textcolor{right}{0.06} & \textcolor{gray}{Commonsense} \\
% & \qquad \textit{Hydrostatic skeletons are a feature of some fish.} & \textcolor{right}{aquatic animals} & \textcolor{right}{0.96} & Induction \\
% \midrule
% \multirow{2}{*}{QASC} & \textbf{[M] requires studying the weather.} & \textcolor{wrong}{research} & \textcolor{wrong}{0.48} | \textcolor{right}{0.43} & \textcolor{gray}{Commonsense} \\
% & \qquad \textit{Meteorology is the study of the weather.} & \textcolor{right}{meteorology} & \textcolor{right}{1.00} & Paraphrasing \\
% \midrule
% \multirow{2}{*}{QASC} & \textbf{Knowledge of the stars can be used for [M].} & \textcolor{wrong}{life} & \textcolor{wrong}{0.63} | \textcolor{right}{0.16} & \textcolor{gray}{Commonsense} \\
% & \qquad \textit{Navigation is when people use the stars to find their way.} & \textcolor{right}{travel} & \textcolor{right}{0.89} & Deduction \\
\bottomrule
\end{tabular}
\caption{
    More examples where prompting with generated knowledge reduces the reasoning type and rectifies the prediction.
    The first row of each section is the original question and the inference results associated with it; the second row is a model-generated knowledge statement that prompts the inference model.
    We show \textcolor{right}{correct answers in green}, \textcolor{wrong}{incorrect answers in red}, and their corresponding scores assigned by the inference model.
}
\label{tab:qualitative_short}
\end{table*}

==> floats/results_qasc_hierarchy.tex <==
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{clc}
\toprule
& \textbf{Knowledge Generation} & \textbf{QASC-dev} \\
\midrule
$\varnothing$ & vanilla baseline & 48.16  \\
$R$ & Random sentences & 48.70 \\
$C$ & Context sentences & 51.30 \\
$K$ & ours & \textbf{58.32} \\
\midrule
$G2$ & Gold separate facts & 76.89 \\
$G1$ & Gold combined facts & 88.55 \\
\bottomrule
\end{tabular}
\caption{
    Performance with different knowledge generation methods.
    Measured on QASC dev set with T5-11b inference model.
}
\label{tab:results_qasc_hierarchy}
\end{table}

==> floats/results_sota.tex <==
\begin{table}[t]
\setlength{\tabcolsep}{3pt}
\footnotesize
\centering
\begin{tabular}{ccccc}
\toprule
& \textbf{Inference} & \textbf{Knowledge} & \textbf{dev} & \textbf{test} \\
\midrule
\multirow{2}{*}{\textbf{NS}} & T5-11b & ours & \textbf{78.0} & \textbf{79.24} | \textbf{72.47} \\
& \multicolumn{2}{c}{Prev. SOTA (no IR)$^*$} & -- & 72.61 | 66.18 \\
& \multicolumn{2}{c}{IR SOTA$^{**}$} & -- & 70.41 | 65.10 \\
\midrule
\multirow{2}{*}{\textbf{CSQA}} & UQA-11b-ft & ours & 85.34 & -- \\
& \multicolumn{2}{c}{Prev. SOTA$^{\#}$} & -- & 79.1 \\
\midrule
\multirow{2}{*}{\textbf{CSQA2}} & Unicorn-ft & ours & \textbf{72.37} & \textbf{73.03} \\
& \multicolumn{2}{c}{Prev. SOTA (no IR)$^\dagger$} & 69.9 & 70.2 \\
& \multicolumn{2}{c}{IR SOTA$^{\dagger\dagger}$} & 74.0 & 73.3 \\
\midrule
\multirow{2}{*}{\textbf{QASC}} & UQA-11b-ft & ours & \textbf{84.02} & \textbf{80.33} \\
& \multicolumn{2}{c}{Prev. SOTA (no IR)$^\ddagger$} & 81.75 & 76.74 \\
& \multicolumn{2}{c}{IR SOTA$^{\ddagger\ddagger}$} & -- & 89.57 \\
\bottomrule
\end{tabular}
\caption{
\hanna{Texts in tables are not well aligned; you should use l (instead of c) for text-based columns Here, you can remove the knowledge column; just use the column as }
    Comparison with state-of-the-art.
    For NumerSense (\textbf{NS}), the test set result consists of two splits: test-core and test-all.
    *: T5-11b 1.1 +digits (Submission by ISI Waltham).
    **: T5-11b + IR \cite{uscink}.
    \#: UQA-11b-ft \cite{khashabi-etal-2020-unifiedqa} (SOTA of single-model methods without referencing ConceptNet).
    $\dagger$: Unicorn-ft \cite{talmor2021commonsenseqa}.
    $\dagger\dagger$: Unicorn-ft + Google snippets \cite{talmor2021commonsenseqa}.
    $\ddagger$: UQA-11b-ft \cite{khashabi-etal-2020-unifiedqa}.
    $\ddagger\ddagger$: UQA-11b-ft + IR \cite{khashabi-etal-2020-unifiedqa}.  \hanna{Not clear if these are fine-tuned or zero shot; also it seems that all the infernece model sizes are similar to your T5-11b, right? then, mention it.}
}
\label{tab:results_sota}
\end{table}

==> floats/results_supervised.tex <==
\begin{table}[t]
\setlength{\tabcolsep}{4pt}
\footnotesize
\centering
\begin{tabular}{clccc}
\toprule
& \textbf{Inference} & \textbf{Knowledge} & \textbf{dev} & \textbf{test} \\
\midrule
\multirow{6}{*}{\textbf{CSQA}} & \multirow{2}{*}{UQA-11b} & -- & 76.99 & -- \\
& & ours & \textbf{78.71} & -- \\
\cmidrule{2-5}
& \multirow{2}{*}{T5-11b-ft} & -- & 83.54 & -- \\
& & ours & \textbf{83.78} & -- \\
\cmidrule{2-5}
& \multirow{2}{*}{UQA-11b-ft} & -- & 85.18 & -- \\
& & ours & \textbf{85.34} & -- \\
\midrule
\multirow{2}{*}{\textbf{CSQA2}} & \multirow{2}{*}{Unicorn-ft} & --$^\dagger$ & 69.9 & 70.2 \\
& & ours & \textbf{72.37} & \textbf{73.03} \\
\midrule
\multirow{6}{*}{\textbf{QASC}} & \multirow{2}{*}{UQA-11b} & -- & 67.93 & 67.07 \\
& & ours & \textbf{74.41} & \textbf{75.33} \\
\cmidrule{2-5}
& \multirow{2}{*}{T5-11b-ft} & -- & 76.03 & 73.91 \\
& & ours & \textbf{78.62} & \textbf{77.17} \\
\cmidrule{2-5}
& \multirow{2}{*}{UQA-11b-ft} & -- & 81.75 & 76.74 \\
& & ours & \textbf{84.02} & \textbf{80.33} \\
\bottomrule
\end{tabular}
\caption{
    Improvement on finetuned models.
    \textbf{-ft}: model finetuned on the corresponding dataset.
    $\dagger$: Unicorn-ft baseline of CSQA2 \cite{talmor2021commonsenseqa}.
}
\label{tab:results_supervised}
\end{table}

==> floats/results_zeroshot.tex <==
\begin{table}[t]
\setlength{\tabcolsep}{4pt}
\footnotesize
\centering
\begin{tabular}{clccc}
\toprule
& \textbf{Inference} & \textbf{Knowledge} & \textbf{dev} & \textbf{test} \\
\midrule
\multirow{4}{*}{\textbf{NS}} & \multirow{2}{*}{T5-11b} & --$^{*}$ & 67.5 & 70.23 | 64.08 \\
& & ours & \textbf{78.0} & \textbf{79.24} | \textbf{72.47} \\
\cmidrule{2-5}
& \multirow{2}{*}{GPT-3} & -- & 72.0 & 74.91 | 66.34 \\
& & ours & \textbf{81.0} & \textbf{80.74} | \textbf{73.46} \\
\midrule
\multirow{2}{*}{\textbf{CSQA}} & \multirow{2}{*}{T5-11b} & -- & 39.89 & -- \\
& & ours & \textbf{47.26} & -- \\
\midrule
\multirow{2}{*}{\textbf{QASC}} & \multirow{2}{*}{T5-11b} & -- & 48.16 & 44.89 \\
& & ours & \textbf{58.32} & \textbf{55.00} \\
\bottomrule
\end{tabular}
\caption{
    Improvement on zero-shot models.
    *: T5-11b baseline on NumerSense \cite{stanford}.
}
\label{tab:results_zeroshot}
\end{table}

==> sections/introduction2.tex <==
\section{Introduction}
\label{sec:introduction}

\input{floats/diagram}
\input{floats/examples}

Commonsense reasoning tasks involve selecting or generating plausible inferences about everyday scenarios \cite{sap-etal-2020-commonsense}.
% Performing commonsense reasoning requires commonsense knowledge.
While pretrained language models implicitly contain a large amount of knowledge and can be directly used for commonsense reasoning \cite{trinh2018simple, yang-etal-2020-designing}, incorporating external knowledge bases (such as ConceptNet \cite{speer2017conceptnet} and ATOMIC \cite{sap2019atomic}) can boost performance on some of these tasks \cite{mitra2019additional, bian2021benchmarking}. 
On the other hand, language models themselves can serve the role as knowledge bases, as they allow for querying knowledge by completing natural language statements \cite{petroni-etal-2019-language, jiang-etal-2020-know}.
To leverage knowledge contained in language models for answering commonsense questions, most recent work manually designs dataset-specific, cloze-style templates to generate certain types of \textit{knowledge statements} (i.e. knowledge expressed as natural language statements), such as clarifications \cite{shwartz-etal-2020-unsupervised} or contrastive explanations \cite{paranjape-etal-2021-prompting}.
% , then conditions on the statements during prediction.
% integrates the knowledge into the inference process.
However, tasks often require different types of knowledge that are beyond the scope of pre-defined templates (\autoref{tab:examples}).
% , and the effect of the mechanism for integrating the knowledge remains unclear.

In this paper, we develop a simple, yet effective, method for eliciting useful knowledge statements from language models and using the knowledge to improve prediction performance. % \hanna{revise the last sentence; similar as the abstract, mention  you generate this knowledge with prompting and demonstration} -- It is mentioned in a later sentence of this paragraph. By the way, I feel that the introduction could be more high-level and we don't necessarily need to give too much details? 
Our method (sketched in \autoref{fig:diagram}, called  \textit{generated knowledge prompting}) consists of two steps%. % uses two language models sequentially: a \textit{knowledge model} and an \textit{inference model}. % \hanna{the phrase our method is kind of overloaded; generated knowledge prompting is the knwoledge model, or the full pipeline?} -- This should be resolved in the current draft, "our method" is the full pipeline; If we need to refer to the knowledge generation only, I would say "our knowledge generation method".
: (1) generating question-related knowledge statements from a language model by conditioning on human-written demonstrations, and (2) using a language model to make predictions with each knowledge statement, then selecting the highest-probability prediction.
% First, we generate question-related knowledge statements from a language model by conditioning on a prompt that contains instructions and few-shot demonstrations. %, which are question-knowledge mappings \hanna{what is question-knowledge mapping? Instead, be more explicit; these demonstrations  are... written by humans for a few examples in each task. Here yo ushould mention that those demonstrations are fixed for each task, and then you are using it for every instance  } written by human.
% These human-written demonstrations show typical questions and helpful knowledge statements for the given task.
% A second language model then uses the generated statements to make a prediction.
% Each knowledge statement is passed to a second language model, which makes a prediction 
% Then we use a second language model to make predictions with each knowledge statement, and select the highest-probability prediction.
% Then, the generated knowledge are integrated into the decision process, where we prompt an inference model with knowledge statements and select the knowledge that maximizes prediction probability.

Experiments show that our method improves both zero-shot and finetuned models on numerical commonsense (NumerSense \cite{lin-etal-2020-birds}), general commonsense (CommonsenseQA 2.0 \cite{talmor2021commonsenseqa}), and scientific commonsense (QASC \cite{khot2020qasc}) benchmarks. % \hanna{cite datasets}
% We take pretrained language models off-the-shelf, use prompts and demonstrations to elicit knowledge statements that transform the commonsense question answering into an explicit reasoning procedure, and prompt the inference model with such knowledge.
% An integration algorithm can adaptively select the best knowledge to inform the decision of inference model.
% This process is unsupervised and resource-efficient, since we do not need a training set to finetune the knowledge generation or inference model, or an in-domain knowledge base to retrieve knowledge from.
% It is also more generic and engineering-efficient compared to previous methods, making it easily adaptable to various tasks.
% 
% We apply our method on recent commonsense reasoning datasets -- NumerSense, CommonsenseQA, CommonsenseQA 2.0, and QASC -- and demonstrate that we can push the limits of existing models.
% Our method improves the state-of-the-art of NumerSense by about 9\%, that of CommonsenseQA 2.0 by about 2\%, and that of QASC by about 3\%.
It shows superior performance over the template-based knowledge generation approach \textit{self-talk} \cite{shwartz-etal-2020-unsupervised}, and 
performs comparably to
% is comparable to and even outperforms 
retrieval-based systems.
% Experimental results show the effectiveness of our method under a variety of settings: with different sizes of inference models, and with both zero-shot and finetuned inference models.
% Notably, it is effective when knowledge generation and inference are done with the same language model.

Our analysis show that three factors contribute to the performance of the generated knowledge prompting method: (i) the \textit{quality} of knowledge -- e.g. our generated knowledge outperforms template-based systems, (ii) the \textit{quantity} of knowledge -- i.e. performance improves with more knowledge statements, and (iii) the strategy for integrating knowledge during inference.
% 
% We identify three factors that contribute to its performance improvements: the high quality of generated knowledge, the large quantity of the knowledge, and the clever selection of good knowledge for inference.
Qualitative analysis suggests that our generated knowledge are of generic types % \hanna{what do you mean by generic types?} -- We defined generic types before, it's one of the desired properties of knowledge and a partial motivation of our method, so I thought we should mention it here.
and can reduce commonsense question answering to explicit reasoning procedures -- e.g. deduction -- that are supported by off-the-shelf and finetuned language models.
% Our work provides a simple recipe for using language models as sources of symbolic knowledge in prediction tasks, and highlights the influence of symbolic knowledge in neural reasoning.
% , and , and we hope that the insights we share will inspire further efforts on neuro-symbolic knowledge integration.
